Simplicity in Auctions Revisited: The Primitive Complexity

In this paper we revisit the notion of simplicity in mechanisms. We consider a seller of $m$ items, facing a single buyer with valuation $v$. We observe that previous attempts to define complexity measures often fail to classify mechanisms that are intuitively considered simple (e.g., the "selling separately" mechanism) as such. We suggest to view a menu as simple if a bundle that maximizes the buyer's profit can be found by conducting a few primitive operations that are considered simple. The \emph{primitive complexity of a menu} is the number of primitive operations needed to (adaptively) find a profit-maximizing entry in the menu. In this paper, the primitive operation that we study is essentially computing the outcome of the "selling separately" mechanism. Does the primitive complexity capture the simplicity of other auctions that are intuitively simple? We consider \emph{bundle-size pricing}, a common pricing method in which the price of a bundle depends only on its size. Our main technical contribution is determining the primitive complexity of bundle-size pricing menus in various settings. We show that for any distribution $\cal D$ over weighted matroid rank valuations, even distributions with arbitrary correlation among their values, there is always a bundle-size pricing menu with low primitive complexity that achieves almost the same revenue as the optimal bundle-size pricing menu. As part of this proof we provide a randomized algorithm that for any weighted matroid rank valuation $v$ and integer $k$, finds the most valuable set of size $k$ with only a poly-logarithmic number of demand and value queries. We show that this result is essentially tight in several aspects. For example, if the valuation $v$ is submodular, then finding the most valuable set of size $k$ requires exponentially many queries (this solves an open question of Badanidiyuru et al. [EC'12]).

==> GS.tex <==

\section{The Main Algorithmic Result: Gross Substitutes Valuations}
\mbc{to be removed!}

\mbc{remark that greedy gives a polynomial upper bound (with value queries only)}

\mbc{move this to a different file and to the appendix for now. } 

In this section, we extend the pivotal idea beyond the algorithm for additive valuations and show algorithms for the two valuation classes of gross-substitutes and budget-additive. 

%We now continue with the class of budget-additive valuations.
%For this class, it is known that the welfare maximization problem cannot be solved for approximation better than $15/16$ using polynomial number of demand queries \rk{\citet{dughmi2015limitations} talk about it but I'm not sure who they are citing, and the lower bound might hold only for deterministic algorithms. or maybe im completely off}. Here we show that the cardinality maximization problem can be solved using polylogarithmic number of demand queries. 

The more \rk{interesting?general? economically motivated? rich? expressiveness?} is the class of gross-substitutes valuation. We extend our results for additive valuations and show an algorithm for gross-substitutes maximization with polylogarithmic query complexity.

\begin{theorem}\label{thm:findmaxkGS}
	Given a gross-substitutes valuation $v$ over a set $\items$ of size $m$, there exists a randomized algorithm that finds a \opt{k} set and has a query complexity of \rk{$polylog m$}.
\end{theorem}

An important characteristic of the class of gross-substitutes valuations is that any \opt{k} set can be achieved via the simple greedy algorithm that adds items of maximal marginal value as long as it is greater than zero, and that solutions are only different by the tie-breaking rule of the greedy algorithm (see \cite{leme2017gross}).
\begin{definition}
    Given a valuation $f$, the {\em greedy ordering} of $f$ over a set $\items$ of size $m$, with a tie-breaking rule $T$, is an ordering $a_1,a_2,\ldots,a_m$ of the items in $\items$ such that for any $i\in[m]$, we have that $a_i\in \arg\max_{x\in \items} f(x|\set{a_1,\ldots,a_{i-1}})$ and the choice of a specific item at each step is according to the tie breaking rule $T$.
\end{definition}

In our setting, Remark 5.5 from \cite{leme2017gross} can be stated as follow:
\begin{claim}\label{cla:greedy}(\cite{leme2017gross}, rephrased)
    Let $f$ a gross-substitutes valuation over $m$ items and $k\in [m]$.
    For any greedy ordering $a_1,a_2,\ldots,a_m$ of $f$, the prefix set $a_1,\ldots,a_k$ is a $\opt{k}$ set. Moreover, for any $\opt{k}$ set $S$, there exists a tie-breaking rule such that $S$ is a prefix of a greedy ordering of $f$.
\end{claim}

\rk{This greedy property guarantees that (up to ties), there exists a price $p$ such that a uniform demand query for this price returns a \opt{k} set (This is not true for general submodular valuations as we later show).
Unfortunately, this is not enough for the previous algorithm to work. Take for example the gross-substitutes valuation with $v(S) = |S|\cdot|S+1|/2$ for any set $S$ of items. For this valuation, the algorithm presented for additive valuations will take a linear number of demand queries regardless of the randomization. The key idea of the improved is that instead of using a random item's value as a pivot, we use a random marginal value by sampling a random set $R$ and a random item $j$ and setting $v(j|S)$ as our pivot.}

before describing the new algorithm, we show how to find efficiently a pair of maximal and minimal sizes sets in the demand for a given price vector. This assists us in handling ties, similarly to the approach taken in the additive case.

Since for any gross-substitutes valuation $v$ and price vector $p$, the valuation $f(S)=v(S)-p(S)$ is also a gross-substitutes valuation, an immediate corollary of claim~\ref{cla:greedy} is that any set in the demand for $p$ is a prefix of a greedy ordering of $f$ such that additional item will cause in a non-positive change in utility.
Hence, by looking at the corresponding ordering and removing all items of zero marginal value, we have that any set in the demand of maximal size contains a set in the demand of minimal size. We now describe an algorithm for finding such a pair.

\begin{lemma}\label{lem:getall}
	Let $v$ a gross-substitutes valuation over a set $\items$. Fix any subset of items $Z\subseteq \items$, a subset $\hat{Z}\subseteq Z$ and $j\in Z\setminus \hat{Z}$.
    Let $B$ be the prefix up to $j$ (exclusive) of some greedy ordering of $v$ over the set $\hat{Z}\cup\set{j}$. Suppose that $v(j|\hat{Z})>0$.
	Let $D'$ be a demand set when setting a uniform price  $p<v(j|\hat{Z})$ for every item $i\in Z$ (and infinity prices for every item $i\notin Z$).
	Then $|D'|>|B|$.
\end{lemma}
\begin{proof}
    Assume by contradiction that $|D'|<|B|+1 = |B\cup\set{j}|$. Then, by Lemma~\ref{lem:S>T}, there exist $t\in (B\cup\set{j})\setminus D'$ such that:
	\begin{equation*}
	v(D')+v(B\cup\set{j})\leq v(D'\cup\set{t})+v((B\cup\set{j})\setminus\set{t}) 
	\end{equation*}
	Rearranging:
	\begin{equation}\label{eq1gseq}
	v(B\cup\set{j}) - v((B\cup\set{j})\setminus\set{t})\leq v(D'\cup\set{t}) - v(D') 
	\end{equation}
	We now have that:
	\begin{eqnarray*}
		p& <    & v(\hat{Z}\cup\set{j}) - v(\hat{Z})\\
		& \leq & v(B\cup\set{j}) - v(B)\\
		& \leq & v(B\cup\set{j}) - v((B\cup\set{j})\setminus\set{t})\\
		& \leq & v(D'\cup\set{t}) - v(D').
	\end{eqnarray*}
	Where the first inequality is by the assumption $v(j|\hat{Z})>0$, the second by submodularity (as $B\subseteq \hat{Z}$), the third is since $B$ created using a greedy ordering of $\hat{Z}\cup\set{j}$ (and hence $v(B)>v((B\cup\set{j})\setminus\set{t})$) $|B|$ and the last by inequality \eqref{eq1gseq}.
	That is, $t$ can be added to $D'$ for price $p$ with positive utility in contradiction to $D'$ being in demand.
\end{proof}


\begin{lemma}\label{lem:getall}
	Given  a gross-substitutes valuation $v$ over a set $\items$ of size $m$, and a price vector $p$, there exists an algorithm with $\O{\log ^2 n}$ query complexity that finds two sets in the demand $D_{min}\subseteq D_{max}$, such that $|D_{max}|$ if maximal over all sets in the demand for price $p$ and $|D_{min}|$ is minimal over all such sets.
\end{lemma}
\begin{proof}
	The algorithm first makes a demand query for $p$. This splits the items into two sets, a set $D$ which is in the demand and $C=N\setminus D$.
    Without loss of generality, we can assume that $p$ is the all-zero price vector by embedding it within $v$ (since $v(S)-p(S)$ is also a gross-substitutes valuation). 
    
    %By Claim~\ref{cla:greedy}, there is a greedy ordering $a_1,\ldots,a_m$  that corresponds to $D$, i.e. $D = \set{a_1,\ldots,a_d}$ and $C = \set{a_{d+1},\ldots,a_m}$.
    %We wish to find a set $A = \set{a_i,\ldots,a_j}$ such that $D_{max} = D\cup A$ and $D_{min} = D\setminus A$.\footnote{Note that there might be several possible such sets. We abuse notation and denote by $A$ any such set.}

	We show how to find $D_{min}\subseteq D$. The algorithm for $D_{max}\supseteq D$ is similar \rk{and is detailed in appendix  XXX}. 
	
    The algorithm works in the following iterative way. Let $D_1$ be a random subset of $D$ of size $k$ (later to be defined), and $j$ a random item from $D\setminus D_1$.
	Assuming $v(j|D_1)>0$, the algorithm makes a demand query with uniform price $\frac{1}{2}v(j|D_1)$ for any item $i\in D$ (and infinity prices for items in $C$) and denote the returned set $D'$.\footnote{Without the assumption that $p$ is suppressed, the algorithm equivalently makes a query with price $p_i+v(j|D_1)/2$ for each item $i\in D$.} 
	
	We denote by $B$ the prefix up to $j$ (exclusive) of a greedy ordering (with random tie-breaking) of $v$ over the set $D_1\cup\set{j}$.
    %In addition, we denote by $G$ the prefix up to $j$ (exclusive) of the greedy ordering of $v(\cdot|R)$ over the set $(\items\setminus R)\cup\set{j}$. In both ordering we assume that ties are broken uniformly at random.
	We now show that $|D'|>|B|$. 
	Assume by contradiction that $|D'|<|B|+1 = |B\cup\set{j}|$. Then, by Lemma~\ref{lem:S>T}, there exist $t\in (B\cup\set{j})\setminus D'$ such that:
	\begin{equation*}
	v(D')+v(B\cup\set{j})\leq v(D'\cup\set{t})+v((B\cup\set{j})\setminus\set{t}) 
	\end{equation*}
	Rearranging:
	\begin{equation}\label{eq1gseq}
	v(B\cup\set{j}) - v((B\cup\set{j})\setminus\set{t})\leq v(D'\cup\set{t}) - v(D') 
	\end{equation}
	We now have that:
	\begin{eqnarray*}
		v(j|D_1)/2& <    & v(D_1\cup\set{j}) - v(D_1)\\
		& \leq & v(B\cup\set{j}) - v(B)\\
		& \leq & v(B\cup\set{j}) - v((B\cup\set{j})\setminus\set{t})\\
		& \leq & v(D'\cup\set{t}) - v(D').
	\end{eqnarray*}
	Where the first inequality is by the assumption $v(j|D_1)>0$, the second by submodularity (as $B\subseteq D_1$), the third is since $B$ created using a greedy ordering of $D_1\cup\set{j}$ (and hence $v(B)>v((B\cup\set{j})\setminus\set{t})$) $|B|$\mbc{unclear} and the last by inequality \eqref{eq1gseq}.
	That is, $t$ can be added to $D'$ for price $v(j|D_1)/2$ with positive utility in contradiction to $D'$ being in demand.
	We have that $\E{|B|} \geq k/2$ since $j$'s location is uniform \mbc{uniform at random?} among all items in $D_1\cup\set{j}$ and thus $\E{|D'|} \geq k/2$. 
	
	\mbc{need to formulate:} By guessing $k$ values ($(2^{-\ell})|D|$) we can find "the best" k to work with (i.e. a maximal one such that $v(j|D_1)$ is still larger than $0$ with good probability). 
	In expectation, after each iteration, $D\D'$ is getting smaller by a factor 2.
	repeating for log n iteration is good enough.


\mbc{Is the next a repeat of the above, or is there anything different?}

    The set $D_{max}$ is handled in similar way.
	The algorithm works in the following iterative way. Let $C_1$ be a random subset of $C$ of size $k$ (later to be defined), and $j$ a random item from $C\setminus C_1$.
	
	Assuming $v(j|D \cup C_1)<0$, the algorithm makes a demand query with uniform (negative) price $\frac{1}{2}v(j|D \cup C_1)$ for any item $i\in C$ (and zero prices for items in $D$) and denote the returned set $D'$. 
	
	we denote by $G$ the prefix up to $j$ (exclusive) of a greedy ordering (with random tie-breaking) of $v(\cdot|D\cup C_1)$ over the set $(C\setminus C_1)$.
	We now show that $|D'|\leq |D\cup C_1\cup G\leq \set{j}|$. 
	
	Assume by contradiction that $|D'|>|D \cup C_1\cup G\cup\set{j}|$. Then, by Lemma~\ref{lem:S>T}, there exist $t\in  D' \setminus (D \cup C_1\cup G\cup\set{j})$ such that:
	
	%Assume by contradiction that $|D'|>|D\cup C_1\cup G|$. Then, by Lemma~\ref{lem:S>T}, there exist $t\in  D' \setminus (D\cup C_1\cup G)$ such that:
	\begin{equation*}
	v(D')+v(D \cup C_1\cup G\cup\set{j})\leq v(D'\setminus\set{t})+v((D \cup C_1\cup G\cup\set{j})\cup\set{t}) 
	\end{equation*}
	Or:
	\begin{equation}\label{eq2gseq}
	v(D') - v(D'\setminus\set{t})\leq v((D \cup C_1\cup G\cup\set{j})\cup\set{t}) - v(D \cup C_1\cup G\cup\set{j})
	\end{equation}
	We now have that:
	\begin{eqnarray*}
		v(D') - v(D'\setminus\set{t})& \leq & v((D \cup C_1\cup G\cup\set{j})\cup\set{t}) - v(D \cup C_1\cup G\cup\set{j})\\
		& \leq & v((D \cup C_1\cup G\cup\set{j})\cup\set{t}) - v(D \cup C_1\cup G\cup\set{t})\\
		& \leq & v((D \cup C_1\cup\set{j}) - v(D \cup C_1) < \frac{1}{2}v(j|D \cup C_1)
	\end{eqnarray*}
	Where the first inequality is by inequality \eqref{eq2gseq}, the second is by the maximality of $R\cup G\cup\set{j}$ over sets of size $|R\cup G\cup\set{j}|$, third by submodularity, and the last is since $v(j|D \cup C_1)<0$.
	That is, $t$ can be added to $D'$ for price $v(j|D_1)/2$ with positive utility in contradiction to $D'$ being in demand.
	That is, $t$ can be removed from $D'$ getting back a price $\frac{1}{2}v(j|D \cup C_1)$ and positive utility, in contradiction to the fact that $D'$ is a set in the demand.
	
	We showed that $|D'|\leq |D\cup C_1\cup G|$. Hence, by the random selection of $j$ we have that $\E{|G|}\leq |D|+k+\frac{|C|-k}{2}$.

	By guessing $k$ values ($(1-2^{-i})|C|$)...
	Assuming $v(a|D \cup C_1)<0$ we are guaranteed that a maximal set of items of marginal zero is added (i.e., some possible set $A$).
	repeating for log n iteration is good enough.

\end{proof}

Next, we cite a Lemma from \cite{kupfer2020adaptive} (for completeness we give a full proof in Appendix~\ref{app:missingproofs}). Intuitively, the Lemma shows an augmentation property similar to the one we have for matroid valuations. 
%This property implies that not only an optimal set, \rk{?} %שניתן להשתמש בקבוצות מקריות יחסית כדי להרחיב פתרון אופטימלי קטן לפתרון אופטימלי גדול
\begin{lemma}\label{lem:S>T}(\cite{kupfer2020adaptive})
%\begin{restatable}[\cite{kupfer2020adaptive}]\label{lem:S>T}
	Given a gross-substitutes function $v$ and two sets $S,T$ s.t. $|S|<|T|$, then $v(S)+v(T)\leq \max_{t\in T\setminus S}\left\lbrace v(S\cup t)+v(T\setminus t)\right\rbrace.$
\end{lemma}

Using this lemma, we are now ready to present our proof for Theorem~\ref{thm:findmaxkGS}.

%\thmfindmaxkGS*
\begin{proof}
	The algorithm works in the following iterative way: at each round, we classify a fraction as the items as desired/undesired items, i.e., either returning a long prefix of the greedy algorithm or ruling out many items as being possibly selected (given the items already chosen).
	
	For each round round, let:
	\begin{itemize}
		\item $R$ - a random set of size $m/2$ chosen uniformly at random
		\item $j$ - an item chosen uniformly at random from $\items\setminus R$
		\item $p = v(R\cup\set{j}) - v(R)$ 
	\end{itemize}
	Next, using Lemma~\ref{lem:getall}, we find two sets in the demand $D_{max}$ and $D_{min}$ for uniform price $p$, such that $D_{min}\subseteq D_{max}$, $D_{max}$ if of maximal size and $D_{min}$ is of minimal size.
    We denote by $B$ the prefix up to $j$ (exclusive) of the greedy ordering of $v$ over the set $R\cup\set{j}$.
    In addition, we denote by $G$ the prefix up to $j$ (exclusive) of the greedy ordering of $v(\cdot|R)$ over the set $(\items\setminus R)\cup\set{j}$. In both ordering we assume that ties are broken uniformly at random.
	
	We first claim that $D_{max}$ is not too small by showing that $|D_{max}|>|B|$.
	
	Assume by contradiction that $|D_{max}|<|B\cup\set{j}|$. Then, by Lemma~\ref{lem:S>T}, there exist $t\in (B\cup\set{j})\setminus D_{max}$ such that:
	\begin{equation*}
	v(D_{max})+v(B\cup\set{j})\leq v(D_{max}\cup\set{t})+v((B\cup\set{j})\setminus\set{t}) 
	\end{equation*}
	Rearranging:
	\begin{equation}\label{eq1gs}
	v(B\cup\set{j}) - v((B\cup\set{j})\setminus\set{t})\leq v(D_{max}\cup\set{t}) - v(D_{max}) 
	\end{equation}
	We now have that:
	\begin{eqnarray*}
		p& =    & v(R\cup\set{j}) - v(R)\\
		& \leq & v(B\cup\set{j}) - v(B)\\
		& \leq & v(B\cup\set{j}) - v((B\cup\set{j})\setminus\set{t})\\
		& \leq & v(D_{max}\cup\set{t}) - v(D_{max}).
	\end{eqnarray*}
	Where the first inequality is by submodularity, the second is by the maximality of $B$ over sets of size $|B|$ contained in $R$ and the last by inequality \eqref{eq1gs}.
	That is, $t$ can be added to $D_{max}$ for price $p$ without harming the utility in contradiction to $D_{max}$ maximality.
	We have that $\E{|B|} = n/4$ since $j$'s location is symmetric among all items in $R\cup\set{j}$ and thus $\E{|D_{max}|} \geq n/4$.

	On the other direction, we similarly show that $D_{min}$ is not too large, namely $|D_{min}|\leq|R\cup G|+1$.	
	
	Assume by contradiction that $|D_{min}|>|R\cup G\cup\set{j}|$. Then, by Lemma~\ref{lem:S>T}, there exist $t\in  D_{min} \setminus (R\cup G\cup\set{j})$ such that:
	\begin{equation*}
	v(D_{min})+v(R\cup G\cup\set{j})\leq v(D_{min}\setminus\set{t})+v((R\cup G\cup\set{j})\cup\set{t}) 
	\end{equation*}
	Or:
	\begin{equation}\label{eq2gs}
	v(D_{min}) - v(D_{min}\setminus\set{t})\leq v((R\cup G\cup\set{j})\cup\set{t}) - v(R\cup G\cup\set{j})
	\end{equation}
	We now have that:
	\begin{eqnarray*}
		v(D_{min}) - v(D_{min}\setminus\set{t})& \leq & v((R\cup G\cup\set{j})\cup\set{t}) - v(R\cup G\cup\set{j})\\
		& \leq & v((R\cup G\cup\set{j})\cup\set{t}) - v(R\cup G\cup\set{t})\\
		& \leq & v((R\cup\set{j}) - v(R) = p
	\end{eqnarray*}
	Where the first inequality is by inequality \eqref{eq2gs}, the second is by the maximality of $R\cup G\cup\set{j}$ over sets of size $|R\cup G\cup\set{j}|$, and the last is by submodularity.
	That is, $t$ can be removed from $D_{min}$ without harming the total utility in contradiction to $D_{min}$ minimality.
	
	We have that $\E{|R\cup G|} = 3/4$  since $j$'s location is symmetric among all items in $R\cup\set{j}$ and thus $\E{|D_{min}|} < 3n/4$.
	
	By submodularity of gross-substitutes valuations, after getting $D_{min}$ and $D_{max}$ we can create a set $D$ such that $D$ is in the demand and $n/4\leq \E{|D_{min}|} \leq 3n/4$ by taking $D_{min}$ and adding any subset of $D_{max}\setminus D_{min}$. Next,
	\begin{itemize}
		\item If $|D|=k$, the algorithm found an optimal set of size $k$.
		\item If $|D|>k$, we know that there is an optimal set of size $k$ contained in $D$ and we can narrow our interest to a smaller item domain $D$ iteratively.
		\item If $|D|<k$, we know that $D$ is a prefix of a greedy algorithm and thus can be extended to an optimal set of size $k$. We keep all $D$ as a desired set and continue iteratively maximizing $v_{D}(\cdot)$ (which is also a gross-substitutes valuation) with the $k-|D|$ cardinality constraint
	\end{itemize}
	Since $\frac{n}{4}\leq \E{|D|}\leq \frac{3n}{4}$, the expected number of iterations is $\O{\log m}$.
\end{proof}


==> discussion.tex <==
\section{Discussion and Further Work}
In this work we showed ccccccc

Open - symmetric auction for iid, symmetric auction for id correlated. How much do you loose?

Open: what is the query complexity of implementing a general symmetric menu? (for additive valuation? At most n, might be polylog as well)


Our results show that is impossible to achieve a $1-1/n$ approximation for submodular maximization under cardinality constraint using polynomial number of demand queries.
\cite{badanidiyuru2012optimization} show an algorithm that achieves a $8/9$ approximation for this problem using polynomial number of queries.
We/they conjuncture that fffffff is tight.

We show that $\sqrt{n}$ queries are needed in the deterministic case. 
It seems that the right bound is linear.
using only value queries requires $n-2$ queries even for the randomized case.\rk{full proof?}


If we assume the distribution over valuations is known, and assuming no ties, the expected number of queries needed in order to find maximal set of size $k$ is in fact constant (where the expectation is over the distribution, the algorithm itself is deterministic). 
\rk{Is it true even with ties? Does it makes theorem \ref{thm:menu_expected} less or more interesting?}

==> hard_menu.tex <==
\subsection{Menus with High Query Complexity}
%\include{hard_menu_old}


In Section~\ref{sec:symmenu} we showed that for additive valuations the implementation complexity of any menu that is based on bundle-size pricing  is poly-logarithmic in the number of items.
We next show that not every menu has such a low implementation complexity: there are menus that are not based on bundle-size pricing that require almost linear
number of demand queries, even when randomization is allowed.

\begin{theorem}
    Let $A$ be a randomized algorithm that -- given an arbitrary menu $M$ -- finds a profit-maximizing bundle of an additive valuation using demand and value queries. The number of queries that $A$ makes is $\Omega(\frac {m} {\log m})$.
\end{theorem}
We prove the theorem by a reduction to the problem of finding a $\frac m 2$-optimal set with value queries. Formally:

\begin{proposition}
    Let $A$ be a randomized algorithm that -- given an arbitrary menu $M$ -- finds a profit-maximizing bundle of an additive valuation using $t$ demand and value queries. Then, there exists an algorithm that finds an $\frac m 2$-optimal set with probability at least $\frac 1 2$ and makes only $O(t)$ value queries.
\end{proposition}
The proposition implies the theorem since we have already established that finding an $\frac m 2$-optimal set with value queries only requires $\Omega(\frac {m} {\log m})$ queries (Proposition \ref{pre:random_lb_additive_information}).

%We accomplish this by presenting a certain menu that ``binds'' pairs of items together and {treats each pair as an item}. We show that in certain distributions demand queries 
%each pair having almost the same total value that is randomly split between the items, 
%cannot benefit from demand queries. As implementation with value queries only require polynomial number of queries even with randomization (Proposition~\ref{pre:random_lb_additive_information}), the results follows.

In fact, we prove the proposition by considering just one specific menu $\menu$ that we now describe. As we will see later, it will be more convenient to think of $\menu$ as a menu for $2m$ items, and not $m$ as usual. $\menu$ is defined as follows: split the items into $m$ disjoint pairs, where every item with an odd index is paired with the item with the next even index (that is, items $\{1,2\}$ are one pair, items $\{3,4\}$ are another, and so on). The price in $\menu$ of every bundle that can be constructed by taking the union of at most $\frac m 2$ of the disjoint pairs is $0$. The price of any other bundle is $\infty$. Note that the profit-maximizing bundle of the buyer is the bundle that consists of the $\frac m 2$ pairs with the highest value.

%for some parameter $k$, the menu
%offers any bundle of $k$ pairs for price zero, and does not offer any larger bundle. 

%We price only the pairs, and the price of bundles that consist of these pairs is additive in the pairs. That is, if the bundle $S$ consists of the pairs $\{x,y\}$ and $\{w,z\}$ then the price of $S$ is the price of $\{x,y\}$ plus the price of $\{w,z\}$. Bundles that contain only one item from a certain pair will be priced $\infty$ in $\menu$.


%Trivially, a buyer wishes to buy exactly $k$ pairs of highest value.
%each for the price of $1+\epsilon$. I.e., it offers for each odd $i$, the  bundle $\{i,i+1\}$ for price $1+\epsilon$. Trivially, a buyer wishes to buy exactly all pairs that their sum of values is at least  $1+\epsilon$.\footnote{The bound is proven for the case that no pair has a value of exactly $1+\epsilon$, so ties are not an issue}.

We now use $A$ to define an algorithm that finds an $\frac m 2$-optimal set with few value queries. Recall that we are given an additive valuation $v$ on $m$ items and we want to find its $\frac m 2$-optimal set. Towards this end, we define a distribution $\Dv$ over additive valuations with $2m$ items, for every $\eps>0$. We will sample a valuation $w$ from $\Dv$ and see that the profit-maximizing bundle of $w$ in $\menu$ is an $\frac m 2$-optimal set of $v$. Thus, our goal is to run $A$ with the input valuation $w$ and the menu $\menu$ to find the profit-maximizing bundle. However, note that we only have access to value queries for the given valuation $v$ and we need to be able to compute both value and demand queries for $w$. We will see that computing value queries for the valuation $w$ is easy to simulate given then we have value query access to $v$. Simulating demand queries for $w$ is harder and is in fact the technical heart of the proof. The success probability of the simulation will depend on $\eps$ and we will show that it goes to $1$ as $\eps$ goes to $0$.

%\sd{rephrase the next sentence -- the success probability depends on $\eps$} We later show that for $\epsilon>0$ that is small enough, any implementation of $\menu$ with $q$ value and demand queries {that succeeds with constant probability} over $\Dv$, 
%can be converted to an algorithm that finds a \opt{k} set using $q$ value queries and has a constant success probability.
%Together with the lower bounds for randomized algorithms that use only value queries shown in Proposition~\ref{pre:random_lb_additive_information}, we establish a polynomial lower bound for finding the profit-maximizing bundle in this menu.

%\mbe{Assume that we are given a parameter $\epsilon>0$ and an additive valuation $v$ over $m$ items such that $v(N)=1$.
%Given $\epsilon$ and $v$, we next define the distribution $\Dv$ over additive valuations.}
% (w.l.o.g. \mbe{we can normalize $v$ such that $v(N)=1$ and thus $v$'s values are bounded in $[0,1]$}).
We now describe how to sample a distribution $w^{u,v}$ from $\Dv$. For simplicity of presentation, we assume without loss of generality that $v(M)=1$. Let $\Um$ be the uniform distribution that samples $m$ i.i.d. values from $[0,1]$. 
We draw $u\sim\Um$ and define the additive valuation $w^{u,v}$ over $2m$ items as follows: $w^{u,v}_{2i-1} = u_i+\epsilon\cdot v_i$ and $w^{u,v}_{2i} = 1-u_i$, for $1\leq i\leq m$.
%We use $\Dv$ to denote the resulting distribution over the additive valuations $w$ sampled using the sampling procedure described above.
Note that the value of the $i$'th pair in $w^{u,v}$ is $w^{u,v}_{2i-1}+w^{u,v}_{2i}=1+\epsilon\cdot v_i$ and thus a profit maximizing set of $w^{u,v}$ in  $\menu$ corresponds to a \opt{k} set of $v$.

%Let $\ALGmenu$ be an algorithm that finds the profit maximizing bundle of $\menu$ and makes both value and demand queries. We construct an algorithm $\ALGvalue$ that finds a \opt{k} set for every additive valuation $v$ using only value queries as follows: we simulate $\ALGmenu$ on a synthetic input $w^{u,v}$ with random $u\sim\Um$.
%Since $\ALGvalue$ can access $v$ using only value queries, it is not immediately clear how to simulate demand queries.
%We next show that the with constant probability the following procedure is consistent with the first $t$ queries made by $\ALGmenu$, where $t$ is a function of $\epsilon$ that goes to infinity as $\epsilon$ approaches zero.  

For every value query for a set $S$ in $w^{u,v}$ that $A$ makes, it is easy to compute $w^{u,v}(S)$, since $u$ is known and a suitable value query to $v$. Computing demand queries is harder. Consider the demand query in which $p_j$ is the price for the $j$'th item (out of $2m$). We wish to find a most profitable set under these prices. Note that $w^{u,v}$ is additive and an item is included in a most profitable set if its value is larger than its price, regardless of the other items.
For an item with even index ($j=2i$), whether the item belongs to a most profitable set is determined by $1-u_i-p_j>0$ and can be computed with no additional queries.
For an item with an odd index ($j=2i-1$), whether the item belongs to a most profitable set is determined by $u_i+\epsilon\cdot v_i-p_j>0$. A naive way to compute the most profitable set is to query the value of each $v_i$ and compute whether the inequality holds. However, this might require querying all the $m$ items. We now present a more efficient method.

Fix some point during the run of $A$. We say that $v_i$ \rk{$u_i$} is {\em determined by previous queries} if the value $v_i$ \rk{$u_i$} is identical in all valuations that are consistent with all queries so far. If $v_i$ is known\rk{$u_i$ is determined}, then whether $u_i+\epsilon\cdot v_i-p_j>0$ can be determined with no additional value queries\rk{using one additional value!}. Else, we will determine whether item $j$ is in the most profitable set assuming that $v_i=0$. That is, we will prove that if $\eps$ is small enough and the number of queries made so far $t$ is small enough as well, then $u_i+\epsilon\cdot v_i-p_j>0 \iff u_i-p_j>0$ with very high probability. Note that the number of value queries to $v$ that needed to simulate $A$ on $w^{u,v}$ is at most the number of demand and value queries that $A$ makes.


%$\ALGvalue$ makes its decision based on $u_i-p_j>0$ without making additional value queries. We observe that $\ALGmenu$ and $\ALGvalue$ make a similar number of queries:
%\begin{proposition}
%    Fix some valuation $v$ and some additive menu. Suppose that $\ALGmenu$ makes $t$ queries when the valuation is $v$ \sd{in expectation? in a specific run of the algorithm?}. Then, for any $u$, $\ALGvalue$ makes at most $2t$ value queries when the input is $w^{u,v}$\sd{on which menu? we somehow need to translate the menu that we started with to the new format -- this probably needs to be defined in the beginning}.
%\end{proposition}
%\begin{proof}
%	Since $u$ is known to $\ALGvalue$, any value query made by $\ALGmenu$ for $w^{u,v}$ is implementable using a single value query for $v$.
%	For the demand queries, the number of value queries done by $\ALGvalue$ is the number of entries of $u$ which are of known value \sd{I don't understand this} in addition to a single value query for the set in demand per query.
%	Since $\ALGmenu$ makes at most $t$ value queries and $u$ is a continuous (and thus is not determined to exact value by demand queries), at most $t$ entries of $u$ are of known value.
%	Hence, $2t$ queries are sufficient for $\ALGvalue$ implementation.
%	\sd{I don't understand this proof, please rewrite}
%\end{proof}

%the answer made by $\ALGvalue$ depends on the \sd{not clear from here until the proposition} information on $u_i$ received from queries done so far.
%If $u_i$ value is determined by previous value queries (i.e. there is only one possible value satisfying the observed linear constraints), the $\ALGvalue$ selects the $j$-th item according to the value $u_i+\epsilon\cdot v_i$. Else, it selects solely according to $u_i$.
%In both cases, after the set $S$ is selected, the returned value $w(S)$ can be found in a single value query for $v$.

%Note that since $u$ is drawn by the algorithm, $\ALGvalue$ only makes value queries accessing $v$.


\begin{proposition}
    Fix $u\in \rke{[0,1]^m}$. Consider a demand query with prices $\vec p$ on $2m$ items and some item $j=2i-1$. If $|p_j-u_i|>\epsilon$ then either item $j$ is in the profit maximizing set of $w^{u,v}$, for every additive valuation $v$ with $v(M)=1$, or $j$ is not in the profit maximizing set of $w^{u,v}$, for every additive valuation $v$ with $v(M)=1$.
\end{proposition}
\begin{proof}
    \rk{trivial?}
\end{proof}

Thus, to complete the proof of the proposition (and thus also the theorem), we will show that after $\frac m {\log m}$ queries, we have with high probability for every item $j$ with an odd index, that in every demand query where the price of item $j$ is $p_j$, either the value of item $j$ is determined by the previous queries or $|p_j-u_i|>\epsilon$. Using the union bound, we will have that demand queries can be computed without making additional queries, since $u_i+\epsilon\cdot v_i-p_j>0 \iff u_i-p_j>0$. 
\rk{additional queries are necessary. assume we queried item $2$. we now have $1-u_1$ and can make a query for item $1$ with $p_1 = u_i+\frac{\epsilon}{2}$.}

\sd{stopped here}


%that with constant probability $\ALGvalue$ agrees with any $\ALGmenu$ for the first $t$ queries, for $\epsilon$ small enough. \sd{where is $t$ defined}
%\rk{What remains to be shown is that whenever $\ALGvalue$ makes a decision based on $u_i-p_j>0$ instead of $u_i+\epsilon\cdot v_i-p_j>0$, the probability of getting the correct is high. I.e., when $u_i$ is not determined by previous queries, with high probability $p_j$ is far from $u_i$.}

%\rk{this is our main claim:}\sd{then write it properly as a lemma}

We now prove that there exists a function $T:\mathbb{N}\times\R_{+}\rightarrow\R_{+}$ such that for any $0<\epsilon<T(t,\delta)$, with probability at least $1-\delta$ (over the choice of $u\sim\Um$), all prices in all queries made by $\ALGmenu$ with input $w^{u,v}$ are at least $T(t,\delta)$ far from $u$ (for all undetermined $u_i$).
Thus, for $\epsilon<T(t,\delta)$ with probability at least $1-\delta$, $\ALGvalue$ can simulate the first $t$ queries made by $\ALGmenu$ regardless of $v$.

We start with a technical claim that shows that in general it is unlikely to guess correctly or even estimate the value of an item.
\begin{lemma}\label{lem:convex2}
    Let $d>0$, and $\F$ be a distribution over additive valuations such that the marginal cumulative distribution function (CDF) of each item is continuous. Then, for every item such that its marginal probability is not a single value, the CDF of $\F$ is a $K$-Lipschitz function, with parameter $K$ that is a function of $\F$. I.e., the marginal probability of the item's  value to be in the sub-segment $[x-d,x+d]$ is at most $2d\cdot K$ for any $x\in\R_{+}$ and $K$ which is a function of $\F$.
\end{lemma}
\begin{proof}
    The marginal CDF $\F$ of each item $i$ is a continuous and bounded function over a compact set and thus is Lipschitz continuous with some finite parameter $K_i$.
    Hence, the probability for $i$'s value to be in any range of width $d$ is $F(x+d)-F(x-d)\leq K_i(x+d-x+d) = 2d\cdot K_i$.
    Taking $K$ to be the maximum $K_i$ over all items concludes our claim. 
\end{proof}

We now prove our main claim.
\begin{lemma}\label{lem:simulation}
    Let $v$ be an additive valuation over $m$ items and $u\sim\Um$.
    There exists a function $T:\mathbb{N}\times\R_{+}\rightarrow\R_{+}$ such that for any $0<\epsilon<T(t,\delta)$, with probability at least $1-\delta$ {over $\Um$}, in any demand query made by $\ALGmenu$ (on the input $w^{u,v}$) with price vector $p$, we have that $|p_j-u_i|>T(t,\delta)$ for all first $t$ queries and $j=2i-1$, \rke{unless $u_i$ is determined}
\end{lemma}
\begin{proof}
    For $t=0$ the claim holds for all $\epsilon>0$ and we can set $T(0,\delta)=1$ for all $\delta>0$.
    Assume by induction that the claim holds for the first $t-1$ queries. I.e., $T(r,\delta)$ is defined for all $r<t$ and $\delta>0$.
    
    We now show how to set $T(t,\delta)$ and consider the $t$'th query made by $\ALGmenu$. Before the $t$-th query, the constraints \sd{what does "constraints" mean?}\rk{the answers returned by previous queries?} \sd{then define the term before using} over $w^{u,v}$ can be represented as a requirement that $w$ follows:
    \begin{itemize}
            \item  $A\vec w=\vec d$ for some $A\in\set{0,1}^{(t-1)\times 2m}$ and $\vec d\in \R^{2m}$ where the $i$'th row represents the value of the $i$'th set returned by a value query. 
            \item $\vec \ell\leq w\leq \vec h$ for $\vec \ell,\vec h\in \R^{2m}$, where $h_i$ is the lowest price for which the $i$'th item is in demand, and $\ell_i$ is the highest price for which the $i$'th item is not in demand.
    \end{itemize}
    We make two conservative assumptions regarding the posterior distribution of $u$ and $v$ after $t-1$ queries:
    \begin{itemize}
        \item Since $w^{u,v}$ is a linear combination of $u$ and $v$, we may assume that the constraint $A\vec w=\vec d$ is given as the constraints $A_v\vec v=\vec d_v$ and $A_u\vec u=\vec d_u$ for suitable $A_v,A_u\in\R^{(t-1)\times m}$ and $d_v,d_u\in\R^{m}$.
        \item By the induction assumption, for $\epsilon<T(t-1,\frac{\delta}{3})$, with probability $1-\frac{\delta}{3}$, the first $t-1$ queries have prices which are at least $T(t-1,\frac{\delta}{3})$ far from $u$.
        Thus, $\vec\ell\leq w\leq\vec h$ can be presented as $\vec\ell_u\leq u\leq \vec h_u$ for suitable $\vec\ell_u , \vec h_u\in \R^m$.
        Moreover, since all prices are at least $T(t-1,\frac{\delta}{3})$ far from $u$, we can round $[\vec\ell_u, \vec h_u]$ in each coordinate to {the largest inner segment who's endpoints are multiplications of $T(t-1,\frac{\delta}{3})$}. That is $\vec\ell'_u = T(t-1,\frac{\delta}{3})\cdot\left\lceil\frac{\vec\ell_u}{T(t-1,\frac{\delta}{3})}\right\rceil$ and $\vec h'_u = T(t-1,\frac{\delta}{3})\cdot\left\lfloor\frac{\vec h_u}{T(t-1,\frac{\delta}{3})}\right\rfloor$.
    \end{itemize}
    
    Thus, the number of all possible $h,\ell$ and $A_u$ to consider is bounded by a function of $t$ and $m$. For fixed $h,\ell$ and $A_u$, the corresponding $d_u$ is then a function of $u$ which independent in $v$ and $\epsilon$.
    
    Observe that since all constraints over $u$ are linear dependencies or range constraints, all the possible posterior distributions for $u$ \rk{cant say non-zero probability} are continuous.
    Hence, by Lemma~\ref{lem:convex2}, for each possible distribution $\F$ and every item which is not determined, there exist $K(\F)$ such that for $x>0$ the probability that $u_i\in [p_j-x,p_j+x]$ is at most $2x\cdot K(\F)$ for any undetermined $u_i$.
    
    For any fixed $h,\ell$ and $A_u$, let $\Du$ be the distribution over distributions over additive valuations with $m$ items, assigning each distribution $\F$ the probability that $\F$ is the posterior distribution for $u$ after $t-1$ queries given $h,\ell$ and $A_u$, where the probability is over $\Um$. \footnote{\rk{$\Du$ is a continuous distribution for any ``reasonable'' definition of continuous set of distributions}} 
    
    Consider the $1-\frac{\delta}{3}$ fraction of distributions {with respect to $\Du$} with lowest parameter Lipschitz constants. Let $K_{\Du}<\infty$ be the suprimum over all $K$ corresponds with those ``good'' distributions. \rk{Note that $K_{\F}$ is upper bounded by any $K'$ of a ``bad'' probability which are all finite.}
    \rke{In the case that any of the ``bad'' distribution is the posterior distribution after $t-1$ queries, we assume the algorithm fails.}
    %For the remaining $1-\frac{\delta}{3}$ fraction of "good" distributions and $x<\frac{\delta}{3mK_{\F}}$ with probability at least $1-\frac{\delta}{3}$ $p_j-$  for all $m$ odd items.
    
    Let $\rho$ be the maximum over all $K_{\Du}$ and let $x=\frac{\delta}{6m\rho}$. Note that this is a maximum over a finite set of finite number and hence $\rho<\infty$. With probability at least $1-m\cdot 2\rho\cdot x=1-\frac{\delta}{3}$ we have that $|p_j-u_i|>x$ for all $j=2i-1$ no matter what are $h,\ell$ and $A_u$.
    
    Setting $T(t,\delta) = \min(x,T(t-1,\frac{\delta}{3}))$, we have that the algorithm fails in the first $t$ steps only it either failed one of the first $t-1$ steps, got a ``bad'' posterior distribution, or we hit a price close to $u_i$ in the $t$-th query even though the a posterior distribution after $t-1$ queries is ``good''.
    We have that the failure probability is at most $\frac{\delta}{3}+\frac{\delta}{3}+\frac{\delta}{3}=\delta$. 
    
    %\rk{probability to last $t-1$ is $>1-\frac{\delta}{3}$. probability to get a good distribution for the $t$-th query is $>1-\frac{\delta}{3}$. probability for our guess to be far in all $m$ odd items is $>1-\frac{\delta}{3}$}
\end{proof}








\cout{

\begin{lemma}
    Let $v$ be an additive valuation over $m$ items and $w\sim\Dv$.
    There exists a function $T:\mathbb{N}\times\R_{+}\rightarrow\R_{+}$ such that for any $0<\epsilon<T(t,\delta)$, with probability at least $1-\delta$ \rke{over $\Dv$}, $\ALGvalue$ has the same output as the first $t$ steps of $\ALGmenu$ with the input $w$.
\end{lemma}
\begin{proof}
    We prove the slightly stronger claim: there exists a function $T(t,\delta)$ such that with probability $1-\delta$, in the first $t$ queries made by $\ALGmenu$, all prices in all demand queries are at least $T(t-1,\frac{\delta}{3})$ far from $u$ (if this is the case, and $\epsilon<T(t-1,\frac{\delta}{3})$ trivially $\ALGmenu$ and $\ALGvalue$ are identical), for $\epsilon<T(t,\delta)$\rk{write cleaner}.

    For $t=0$ the claim hold for all $\epsilon$ and we can set $T(0,\delta)=1$ for all $\delta>0$.
    Assume by induction that for the first $t-1$ the claim holds. I.e., $T(r,\delta)$ is defined for all $r<t$ and $\delta>0$.
    
    We now show how to set $T(t,\delta)$ and consider the $t$-th query made by $\ALGmenu$. %
    %If the $t$'th query is a value query, the algorithm always returns a consistent answer and this case does not affects $T(t)$.
    
    %Let $p^t$ and $D_t$ be the price vector and returned set of the $t$'th demand query, respectively.
    %The two constraints observed by the query are:
    %\begin{enumerate}
    %    \item $D_t$ is a set in demand for price vector $p^t$. \rke{In this context we refer to this for of constraint as demand constraint.}
    %    \item $v(D_t)=d_t$ for some value $d_t$. \rke{In this context we refer to this for of constraint as value constraint.}
    %\end{enumerate}
    For any item $j$ let $p_j$ its price in the $t$-th demand query.
    For $j=2i$, the inclusion of the item in a demand set depends only $u_i$ and thus always consistent with the algorithm decision.
    For $j=2i-1$, unless $u_i$ is in the sub-segment $[p_j-\epsilon,p_j]$, answering according to $u$ is consistent with answering the demand query on $w$. We now make sure that $\epsilon$ is small enough to ensure that this is indeed the case for all odd items with constant probability.
    
    Before the $t$-th query, the constraints over $w$ can be represented as a requirement that $w$ follows:
    \begin{itemize}
            \item  $A_t\vec w=\vec d^t$ for some $A_t\in\set{0,1}^{(t-1)\times 2m}$ and $\vec d^t\in \R^{2m}$ where the $i$'th row represents the value of the $i$'th set returned by a query. 
            \item $\vec \ell^t\leq w\leq \vec h^t$ for $\vec \ell^t,\vec h^t\in \R^{2m}$, where $h^t_i$ is the lowest price for which the $i$'th item is in demand, and $\ell^t_i$ is the highest price for which the $i$'th item is not in demand.
    \end{itemize}
    We make the conservative assumption that the constraint $A_t\vec w=\vec d^t$ gives both the constraint $A_t\vec v=\vec d_v^t$ and $A_t\vec u=\vec d_u^t$ such that $\vec d_v^t+\vec d_u^t =\vec d^t$.
    By the induction assumption, for $\epsilon<T(t-1,\frac{\delta}{3})$, with probability $1-\frac{\delta}{3}$, the first $t-1$ demand sets can be found independently of the realization of $v$ and thus $\vec\ell^t\leq w\leq \vec h^t$ can in fact be presented as $\vec\ell_u^t\leq u\leq \vec h_u^t$ for suitable $\vec\ell_u^t , \vec h_u^t\in \R^m$.
    \rk{Moreover, by the induction assumption we have that $\vec\ell_u^t$ and $\vec h_u^t$ are at least $T(t-1,\frac{\delta}{3})$ far from $u$ in all coordinates. Hence, we can make the conservative assumption that $\vec\ell_u^t$ and $\vec h_u^t$ are rounded to the nearest $T(t-1,\frac{\delta}{3})$ multiplication. I.e. $\vec\ell_u^t = T(t-1,\frac{\delta}{3})\cdot\left\lceil\frac{\vec\ell_u^t}{T(t-1,\frac{\delta}{3})}\right\rceil$ and $\vec h_u^t = T(t-1,\frac{\delta}{3})\cdot\left\lfloor\frac{\vec h_u^t}{T(t-1,\frac{\delta}{3})}\right\rfloor$.}
    
    Let $\F$ be the distribution over distributions over additive valuations with $m$ items, assigning each distribution $\D'$ the probability that $\D'$ is the posterior distribution for $u$ after $t-1$ queries, where the probability is over $\D$ and the random decisions made by the implementation. 
    %\rk{This implementation is for specific $\De$. However, since XXXXXXXX we can take a worst case over the finite number of queries (as a function of $m,t$ and $\delta$) which is independent in $\epsilon$ (since we rounded the demand queries and there are only $2^m$ possible value queries). Thus we only need to consider a finite number of $\F$.}
    
    Observe that since all constraints on $u$ are linear or range constraints, all the possible posterior distributions for $u$ \rk{cant say non-zero probability} are continuous.
    Hence, by Lemma~\ref{lem:convex2}, for each possible distribution $\F$ and every item which is not determined, there exist $K(\F)$ such that the probability that $u_i\in [p_j-\epsilon,p_j]$ is at most $\epsilon\cdot K(\F)$.
    Consider the $1-\frac{\delta}{3}$ fraction of distributions {with respect to $\F$} with lowest parameter Lipschitz constants. Let $K_{\F}<\infty$ be the suprimum over all $K$ corresponds with those distributions. \rk{Note that $K_{\F}$ is upper bounded by any $K'$ of a ``bad'' probability which are all finite.}
    If any other distribution is the posterior distribution after $t-1$ queries, we assume the algorithm fails.
    For the remaining $1-\frac{\delta}{3}$ fraction of distributions and $\epsilon<\frac{\delta}{3mK_{\F}}$ with probability at least $1-\frac{\delta}{3}$ the algorithm answers correctly for all $m$ odd items.
    
    \rke{We now define $\rho$ as maximum over all $K_{\F}$. Note that since we assume that demand prices are rounded to a multiplication of $T(t-1,\frac{\delta}{3})$, there are finite number of possible queries (as a function of $m,t$ and $\delta$) and all answers (i.e., $A_t$ and $\vec d_u^t$) are independent of $\epsilon$. Thus we only need to consider a finite number of $\F$.}
    
    We have that the algorithm fails in the first $t$ steps only it either failed one of the first $t-1$ steps, got a bad posterior, or we hit a price close to $u_i$ in the $t$-th query.
    By setting $T(t,\delta)=\min\set{T(t-1,\frac{\delta}{3}),\frac{\delta}{6m\rho}}$, we have that the failure probability is at most $\frac{\delta}{3}+\frac{\delta}{3}+\frac{\delta}{3}=\delta$. 
    
    \rk{probability to last $t-1$ is $>1-\frac{\delta}{3}$. probability to get a good distribution for the $t$-th query is $>1-\frac{\delta}{3}$. probability for our guess to be far in all $m$ odd items is $>1-\frac{\delta}{3}$}
\end{proof}

}







Using Lemma~\ref{lem:simulation}, we conclude that for  some distribution over additive valuations the implementation complexity of $\menu$ must be almost linear (note that a linear implementation is trivial, by a value query for each item). \sd{if we concluded that the implementation is linear, why do we need a proof for the next theorem?}

\begin{theorem}
    $\menu$ implementation complexity is $\Om{\frac{m}{\log m}}$.
\end{theorem}
\begin{proof}
    Let $v$ be an additive over $m$ items.
    Assume that for all $\epsilon>0$ there is an implementation of $\menu$ for $\Dv$ that uses $o(\frac{m}{\log m})$.
    For $\epsilon<T(\frac{m}{\log m},\frac{1}{2})$ we have that the algorithm with parameter $\epsilon$ finds a \opt{k} set with constant probability using $o(\frac{m}{\log m})$ value queries, in a contradiction to Proposition~\ref{pre:random_lb_additive_information}.\sd{I'm sure that we can prove the theorem directly, without assuming towards contradiction}
\end{proof}

\rk{Remark: a more realistic menu will be the additive menu the offers any pair for price $1+\frac{\epsilon}{2}$. This menu has the same implementation complexity and the proof is identical.} \mbc{I guess that by "realistic" you mean "revenue maximizing" (up to epsilon). I agree that this is more attractive (our current one maximizes welfare, but the trivial mechanism that gives everything for free also does that.)}

\rk{We consider in this section implementations of a menu with constant success probability. In general we not consider such implementations since failing possibility may effects incentive compatibility. This is not an issue when discussing lower bounds.}

==> hard_menu_old.tex <==
\subsection{Menus with High Query Complexity}
%Overview:
%In this work we suggested that query complexity is a good measure for the simplicity of an auction and show that \rke{some intuitive menus} are "simple" in that sense. 
\mbc{revise this section!}

We have shown that implementing a \emph{symmetric} menu for additive valuations has low (poly-logarithmic) query complexity. We next show that some \emph{non-symmetric} menus 
require polynomial number of demand queries, even when randomization is considered.
%Note that our lower bound for finding \opt{k} set over submodular valuations gives an exponential bound for the query complexity of auction over this class of valuations.

%Since we discuss only additive valuations in this section, we abuse notation and sometimes refer to additive valuations as vectors in $\R^m$.

Consider the menu $\menu_\epsilon$ that sells $m$ items (with even $m$)
in $\frac m 2$ pre-paired pairs, each for the price of $1+\epsilon$. I.e., it offers for each odd $i$, the  bundle $\{i,i+1\}$ for price $1+\epsilon$. Trivially, a buyer wishes to buy all pairs that their sum of values is at least  $1+\epsilon$ \mbc{need to be careful about ties. Maybe say that the bounds is proven for the case that no pair has a value of exactly $1+\epsilon$, so ties are no an issue}.

To show that $\menu_\epsilon$ cannot be efficiently implemented using any randomized algorithm, we use Yao's principle and describe a distribution $\D$ over valuations such that no deterministic algorithm could succeed with a constant probability when the inputs are distributed according to $\D$. 

\mbc{here is a suggested new proposition (to replace the lemma)}

\begin{proposition}
    Consider the menu $\menu_\epsilon$ over $m$ items for $\epsilon>0$ that is small enough. There exists a distribution $\D$ over additive valuations such that any deterministic algorithm that makes $t=o\left(\frac {m}{\log m}\right)$ demand queries,  fails with probability at least half to implement the menu on a valuation drawn from $\D$.
    %For any number of items $m$, for any small enough $\epsilon>0$ such that any \mbc{deterministic?} algorithm that makes $t=o\left(\frac {m}{\log m}\right)$ demand queries fails to implement $\menu_\epsilon$ over $m$ items who's values drawn from $\D$ with constant probability.
\end{proposition}
In the rest of this section we prove the proposition. 

Let $\D_a$ be the following distribution over additive valuations:
we draw $\frac m 2$ values $a_1,\ldots,a_{\frac m 2}$, independently and uniformly from $[0,1]$, and define $\vec v^a = \left(a_1,1-a_1,\ldots,a_{m/2},1-a_{m/2}\right)\in \R^m$. The valuation $v^a$ for a set $S$ is then $v^a(S)=\sum_{i\in S} \vec v^a_i$. \mbc{need to rewrite this - this notation of $a_i$ does not include even elements. so we need the odd elements to be picked, and even elements be one minus the prior odd element. }

Let $\D_b$ be the following distribution over additive valuations:
we choose uniformly at random $\frac m 4$ of the $\frac m 2$ pairs,\mbc{to make sure we learn nothing from one to the other, we need to pick each with probability half, independently.
might need to adjust Proposition~\ref{pre:random_lb_additive_information}  to match any change here.} 
and give each one of the items in a chosen pair an additional \mbc{why "additional"?} value of $\epsilon$. That is, $\vec v^b = (b_1,\ldots,b_m)\in \R^m$, is the vector where $b_{2i-1} = b_{2i}=\epsilon$ if the $i$'th pair was chosen, and $b_{2i-1} = b_{2i} = 0$ otherwise. The valuation $v^b$ for a set $S$ is then $v^b(S)=\sum_{i\in S} b_i$.

Finally, $\D$ is distribution that samples $v^a\sim \D_a$ and $v^b\sim \D_b$, and returns a valuation $v$ such that $v(S)=v^a(S)+v^b(S)$.
%We abuse notation and refer to $v$ as a pair $(v^a,v^b)$.
Note that the sum of values in each pre-paired pair is either $1$ or $1+2\epsilon$, for all valuations in the support of $\D$, and that the $i$'th pair is bought if and only if $v^b_i=\epsilon$.

%first, we draw $\frac m 2$ values $a_1,\ldots,a_{m/2}$, independently and uniformly from $[0,1]$. Let $\vec a = \left(a_1,1-a_1,\ldots,a_{m/2},1-a_{m/2}\right)\in \R^m$.
%We then choose uniformly at random $m/4$ of the $m/2$ pairs, and give each one of the items in a chosen pair an additional value of $\epsilon/2$. Formally, let $\vec b \in \R^m$, be a vector where $b_{2i-1} = b_{2i}=\epsilon/2$ if the $i$'th pair was chosen and $b_{2i-1} = b_{2i} = 0$ otherwise, and the final valuation $v$ is the additive valuation defined by $v_i = a_i+b_i$. 


%We claim that with high probability, demand queries only give information over the valuation $v^a$ which is irrelevant for the buyer decision.

%Any demand query that prices an item $i$ with $p_i$ such that $|p_i-v^a_i|>\epsilon$, returns the same set in demand $D$ regardless of the realization of $v^b$. 
%In this case the constraint of $v^b$ is only for the value $v^b(D)$.
%does not disclose information over $v^b_i$ other than
%the value of the returned set, which is no more information than an explicit two value queries over the valuations $v^a$ and $v^b$ separately.
%On the other hand, pricing an item $i$ with $p_i$ such that $|p_i-v^a_i|<\epsilon$ requires a good estimation of $v^a_i$ to begin with, which in turn requires either querying for exact value, or having estimation of $v^a_i$ up to accuracy that depends in $\epsilon$.
%polynomial number of queries with high probability.

%That is, finding maximal-profit set depends only on the values in $v^b$ which with high probability can be accessed only through value queries. As shown in Section~\ref{sec:value_lb}, $\Om{m/\log m}$ value queries are required. 
%We now prove this intuition formally. 
%In the proof we abuse notation and refer to $v$ as a pair $(a,b)$ of two additive valuations such that $v(S)=a(S)+b(S)$, $a(S)=\sum_{i\in S} a_i$ and $b(S)=\sum_{i\in S} b_i$.

\begin{lemma}
    For any number of items $m$, for any small enough $\epsilon>0$, any \mbc{deterministic?} algorithm that makes $t=o\left(\frac {m}{\log m}\right)$ demand queries fails to implement $\menu_\epsilon$ over $m$ items who's values drawn from $\D$ with constant probability. \sd{$\eps$ is not in the statement??}\rk{in the definition of $\menu_\epsilon$}
    %Fix an algorithm $A$ that finds the maximum profit bundle in $\mathcal M$ when the distribution is drawn from $\D$. $A$ makes in expectation $\Om{m/\log m}$ value and demand queries.
    % \mbc{here is a suggested new version:}
\end{lemma}
\begin{proof}
    Let $p^r$ and $D_r$ be the price vector and returned set of the $r$'th demand query, respectively.
    The two constraints observed by the query are:
    \begin{enumerate}
        \item $D_r$ is a set in demand for price vector $p^r$. \rke{In this context we refer to this for of constraint as demand constraint.}
        \item $v(D_r)=d_r$ for some value $d_r$. \rke{In this context we refer to this for of constraint as value constraint.}
    \end{enumerate}
    
    After $t$ queries, the constraints over $v$ can be represented as a requirement that $v$ follows:
    \begin{itemize}
            \item  $A_t\vec v=\vec d^t$ for some $A_t\in\set{0,1}^{t\times m}$ and $\vec d^t\in \R^m$ where the $i$'th row represents the value of the $i$'th set returned by a query. 
            \item $\vec \ell^t\leq v\leq \vec h^t$ for $\vec \ell^t,\vec h^t\in \R^m$, where $h^t_i$ is the lowest price for which the $i$'th item is in demand, and $\ell^t_i$ is the highest price for which the $i$'th item is not in demand.
    \end{itemize}
    We make the conservative assumption that the constraint $A_t\vec v=\vec d^t$ gives both the constraint $A_t\vec v^a=\vec d_a^t$ and $A_t\vec v^b=\vec d_b^t$ for some vectors such that $\vec d_a^t+\vec d_b^t =\vec d^t$. 
    %(Since $\vec a$ and $\vec b$ are drawn independently, the constraint $A_t\vec b=\vec d_b^t$ is the only one relevant for the values of $b$.)

    Let $T_t$ be the set of items for which $v^b_i$ is not determined\rk{fixed?computable?} by the constraint $A_t\vec v^b=\vec d_b^t$.
    %with accuracy less than $2^{-m^{2}}$. I.e. $i\in T_t$ if $\max_{\vec v\in\set{\vec v'\R^m|A_t\vec v'=\vec d^t}}v_i - \min_{\vec v\in\set{\vec v'\R^m|A_t\vec v'=\vec d^t}}v_i \geq 2^{-m^{2}}$ 
    
    We first claim that for small enough $\epsilon$, % \mbe{after $t$ queries} 
    with probability $1-3mt\cdot 2^{-m}$, the identity of the set returned for all $t$ demand queries is a function of $v^a$, and is not effected by the realization of $v^b$. \sd{what does that mean??}\rk{rephrased. I.e., the demand constraints are determined by $v^a$.}

    \begin{claim}
        For every $m$ and $t$, there exists $\epsilon'>0$, such that for any $\epsilon<\epsilon'$ with probability $1-3tm^2\cdot2^{-m}$, for any of the first $r\leq t$ queries, and any item $i\in T_t$, we have that $|p^r_i-v^a_i|>\epsilon'$ \rk{Hence, the set returned in demand query for $v$ and $v^a$ using the same price vector is the same \rke{and also $|h^{t}_i-\ell^{t}_i|>\epsilon'$}}.\sd{should be that item $i$ is either in the demand sets of the query on $v$ and $v^a$ or not in both -- currently the claim requires consistency also for items that are not in $T_t$}
    \end{claim}
    \begin{proof}
        %Since there are known dependencies between different items (e.g., $\Pr(v_0+v_1=1)=\frac{1}{2}$), we make the conservative assumption that the fact that item $j$ is or is not in demand introduces a new range constraint on $i$, and there are $m$ prices introduced per item in each query.
        For $\epsilon'<2^{-m}$, for all $i\in T_0$, with probability at least $1-2\cdot 2^{-m}$, a price $p^0_i$ is not in $\epsilon'$ environment of $v^a_i$, i.e., $|p^0_i-v^a_i|>\epsilon'$.
        Summing over all prices and items gives that with probability at least $1-2m\cdot2^{-m}$, this hold for all items in $i\in T_0$.
        
        Assume the claim is true for $t$ and consider the $t+1$'th query. \mbc{isn't the proof by induction on $r$?}
        
        We first observe that for any item $i\in T_{t}$, the value of $v^a_i$ is not determined by the constraint $A_t\vec v^a=\vec d_a^t$.
        \rk{is it trivial? This is since $v^b_i$ is not determined, and $v^b_i$ is determined only if $e_i$ is dependent in the rows of $A_t$, which is the same for $v^a$} \mbc{not exactly as if $i$ is odd, getting $e_{i+1}$ is as good.}
        %Since $v^a$ distribution is continuous and independent in $\epsilon$,
        
        
        %For $i\in T_t$, let $\mu_i=\E{v^a_i|A_t\vec v^a=\vec d_a^t,~ \rke{\vec \ell^t\leq v\leq \vec h^t ?}}$.
        
        %Let $c_t$ be the maximal value such that $\sum_{j\in T_{t-1}}\Pr(|v^a_j-\mu_j|>c_t)>1-2^{-m^2}$. \rk{(expectation given value and constraints...)} Since $v^a_j$ is not determined for any $j\in T_t$, we have that $c_t>0$ and since $v^a$ is independent in $\epsilon$, so is $c_t$.
        %Let $C_t$ the event that for all items are in $c_t$.
        %For $\epsilon<c_t$, any constraint is solvable with any assignment for $v^b$.
        
        \mbc{we need to show that if $i\in T_t$ then $h^{t}_i-\ell^{t}_i$ is large compared to $\epsilon'$. That is, we need to prove the following claim: "For $\epsilon=XYZ$ it holds that $h^{t}_i-\ell^{t}_i\geq \epsilon 2^m"$. Moreover, the posterior distribution (given all prior queries) on the interval is "close to uniform". One observation: I think the distributions are continuous on compact sets, so the derivative is bounded. Can we use this? }
        
        Any range $[\ell^{t}_i,h^{t}_i]$ can be divided into $2^{m}$ subranges of equal probability \mbc{why equal? this needs a proof}.
        Let $r_t$ be the minimal width of any subrange for any $i$, \rke{for specific values of $h^t,\ell^t,A_t$ and $d_a$}. Since $v^a_i$ is continuous and undetermined, $r_t>0$.\rk{how to say explicitly: there is $x$ such that with probability $1-2^{-m}$ (over $v^a$, and under the induction assumption (that removes dependencies in $\epsilon$)), $r_t>x$ and we take $\epsilon<<x$?} 
        
        For any $i\in T_t$, the probability that $p_i$ to be is in the same subrange as $v_i$, or one adjacent to it, is $3\cdot 2^{-m}$.
        Summing over all items gives that with probability at least $1-3m\cdot 2^{-m}$ all prices are at least \rke{x} away from $v^a$ and the claim holds.
    \end{proof}
    

    Taking $\epsilon'<\min_{t'\leq t+1}r_t$, guarantees that after $t$ queries, with probability \rk{$XXXX$}, all of the constraints on $v^b$ are captured by the linear system $A_t\vec v^b=d_b$.

    %for any $i\in T_t$, a random guess will miss $v_i$ by more than $\epsilon$ with probability $1-mt2^{-m^2}$. \rke{hence only linear constraints are interesting.}

    %We make the conservative assumption that the constraint $A_t\vec v=\vec d^t$ gives both the constraint $A_t\vec a=\vec d_a^t$ and $A_t\vec b=\vec d_b^t$ for some vector such that $\vec d_a^t+\vec d_b^t =\vec d^t$. Since $\vec a$ and $\vec b$ are drawn independently, the constraint $A_t\vec b=\vec d_b^t$ is the only one relevant for the values of $b$.
    Let $b'$ be the valuation $v^b$ restricted to the first item from each pair.
    The above implies that all the constraints on $b'$ are in fact implementable using value queries. \sd{I don't understand this argument.}
    The distribution of the valuation $b'$ is the same as in Proposition~\ref{pre:random_lb_additive_information} for $m/2$ items, which implies that for $t=o({m/\log m})$ any algorithm fails to find a most profitable set.\rk{alternatively, we can set $b'$ distribution to proposition 4.11, or any other "hard for value queries" dist.}
\sd{The last paragraph is not clear and not formal. The proof structure seems to be the following: we can take an instance of the hard distribution of claim C.9, split it to obtain the distribution of this claim, and simulate a run of the algorithm on the distribution of the current claim with demand queries using only value queries on the hard distribution of C.9 such that if the algorithm succeeds on the current distribution it succeeds on the distribution of C.9 with approximately the same probability.}
\end{proof}

%\rk{Note that we could use Proposition~\ref{pre:random_lb_additive_DISJ} to choose values for $b$ such that finding a single maximal pair still requires $\Om{n/\log n}$ value queries.}


==> lb_deterministic.tex <==
\subsection{Proof of Theorem \ref{thm-deterministic}}
\label{app:det-lb}

Since we discuss only additive valuations in this section, we abuse notation and sometimes refer to additive valuations as vectors in $\R^m$, with each element representing the value of the corresponding item.

We start with several lemmas regarding linear constraints that will be useful in the proof. First, recall that {\em basic feasible solutions (BFS)} are non-negative solutions to a linear system with minimal support (see, e.g., \cite{eisenbrand2006caratheodory,matousek2007understanding}).%, to deduce that when having less than $m$ linear constraints, many of the items still might have a zero value.

\begin{lemma}[\cite{matousek2007understanding}]\label{lem:sparse}
	For $A\in \R^{\ell\times m}$ and $b\in \R^{\ell}$, if the system ($Ax=b$, $x\geq 0$) has a solution, it has a solution with support of size at most $\ell$.
\end{lemma}

%Having items with value exactly zero could be problematic when constructing a hard valuation, since any one of them is of minimal value. We now exploit the continuity in the set of solutions (for a specific set of equations) to find a set which is arbitrarily close to a BFS but all entries of $v$ are strictly positive.
\begin{claim}\label{pro:continuance}
    Let $\alpha,\beta\in \R$ such that $\alpha+\beta=1$.
	If $\vec x$ is solution of the linear system $A\cdot v=A\cdot\vec{\textbf{1}}$, then so is $y = \alpha\cdot \vec x + \beta \cdot \vec{\textbf{1}}$.
\end{claim}
\begin{proof}
Since both $\vec x$ and $\vec{\textbf{1}}$ are solutions of the linear system $A\cdot v=A\cdot\vec{\textbf{1}}$, we have that 
$$A\cdot y=A\cdot (\alpha\cdot\vec  x + \beta\cdot \vec{\textbf{1}})=\alpha \cdot A\cdot\vec  x +\beta \cdot A \cdot \vec{\textbf{1}} =(\alpha+\beta)\cdot A\cdot\vec{\textbf{1}}=A\cdot\vec{\textbf{1}}$$
\end{proof}

\begin{lemma}\label{lem:n_value_queries}
    Let $A\in \R^{\ell\times m}$ be a matrix of rank at most $m-1$.
	The linear system $A\cdot v=A\cdot\vec{\textbf{1}}$ with the constraint $v\geq 0$ has two different solutions which disagree on the identity of the item with the smallest value.
\end{lemma}
\begin{proof}
	The vector $\vec{\textbf{1}}$ is a solution. In addition, since $A$'s rank is smaller than $m$, there exists some solution $w\in\R^m$ such that $w$ and $\vec{\textbf{1}}$ are independent. Let $\vec x = (1-\epsilon)\vec{\textbf{1}} + \epsilon\cdot \vec w$ and $\vec y = (1+\epsilon)\vec{\textbf{1}} - \epsilon\cdot \vec w$ for a small enough $\epsilon>0$ to ensure that all entries in $\vec x$ and $\vec y$ are positive. 
	Note that by Claim \ref{pro:continuance} both $\vec x$ and $\vec y$ are solutions of the linear system.
	The values in $\vec{x}$ and $\vec{y}$ are ordered according to $\vec{w}$ where a minimal item in $\vec{x}$ is maximal and $\vec{y}$ and vice versa. 
	Since $\vec{w}$ is not the all zero vector, these two solutions disagree on the identity of the items with the smallest value.
\end{proof}

%For additive valuations, we can assume with a small loss in the generality, that there are no demand queries mixing zero and non-zero prices in the same query. This is true since we can replace every demand query with $0$ prices with two queries: one is a value query for all the items that have a price of 0, and a second query with the original non-zero prices and a replacement of every 0 price with a large enough price (the sum of all items can be found in a single query).



We are now ready to prove Theorem \ref{thm-deterministic}.
Throughout the proof, we assume that in all demand queries that $A$ makes the prices are strictly positive. This assumption only doubles the number of queries: if there is a demand query that gives $0$ prices for some set of items $S$, we can replace all $0$ prices with $\infty$, run the new demand query and return the union of $S$ and the answer $T$ of the new demand query. Since the demand query should also return the value of $S\cup T$ we can make one value query $v(S)$ and return $v(S)+v(T)$ (recall that a demand query also returns the value of the most demanded set).


\begin{proof}[of Theorem \ref{thm-deterministic}]
We show that for every deterministic algorithm $A$ there is an adversary that can answer all queries in a way in which after $o(\sqrt m)$ queries there are two different valuations $v,v'$, both consistent with the queries asked, but $\arg\min_jv(j) \neq \arg\min_jv'(j)$. Thus, the algorithm does not distinguish between $v$ and $v'$ and does not find an $(m-1)$-optimal bundle.

We will describe a set  of valuations and show by induction that every valuation that is in this set is consistent with the queries asked so far. Thus, every item that is a minimal item of a valuation in the set is a possible solution. We will need the following notation: for each $i$, let $t_i$ be the number of value queries asked before the $i$'th demand query. 

\begin{claim}\label{claim-invariant}
Consider an execution of the algorithm after a set of $\mathcal Q$ queries. Let $t_{r}$ denote the number of value queries made before the $r$'th demand query in $\mathcal Q$. Suppose that $\mathcal Q$ contains $i$ demand queries and $x$ value queries. Let $x'$ denote the number of value queries made after the last ($i$'th) demand query. There exists an adversary, a non-empty set of valuations $\mathcal V^{\mathcal Q}$, a set of items $L^{\mathcal Q}\subseteq \items$ where $|L^{\mathcal Q}|=\sum_{r\leq i}t_{r}$, a matrix $A^{\mathcal Q}\in \set{0,1}^{(t_i+x')\times (m-|L^{\mathcal Q}|)}$ and $\epsilon^{\mathcal Q}>0$ such that:
\begin{itemize}
    \item All valuations in $v\in \mathcal V^{\mathcal Q}$ are consistent with the queries so far.
    \item For each $v,v'\in \mathcal V^{\mathcal Q}$ and $j\in L^{\mathcal Q}$, $v(\{j\})=v'(\{j\})$.
    \item By renaming, assume without loss of generality that the items that are not in $L^{\mathcal Q}$ are indexed $1,\ldots, m-|L^{\mathcal Q}|$. For each $v\in \mathcal V^{\mathcal Q}$ it holds that:
        \begin{equation*}
            A^{\mathcal Q}\cdot v = \epsilon^{\mathcal Q}\cdot A^{\mathcal Q}\cdot \vec{\textbf{1}}
        \end{equation*}
\end{itemize}
\end{claim}
\begin{proof}
We prove the claim by induction over the number of queries. The base case is when $\mathcal Q$ is the empty set, before the algorithm makes any queries. Let $L^{\mathcal Q}=\emptyset$, $\epsilon^{\mathcal Q}=1$, and $A^{\mathcal Q}$ which is null. The claim trivially holds for this case.

%We now show that for every value query made after the $i$'th demand query and before $(i+1)$'th demand query, these invariants are preserved.
We now assume the induction hypothesis for $\mathcal Q'$, and prove for $\mathcal Q$, where $\mathcal Q$ is $\mathcal Q'$ with an additional query. We describe how the adversary answers the additional query and how to obtain $A^{\mathcal Q}$, $L^{\mathcal Q}$, $\epsilon^{\mathcal Q}$, for which the claim holds after each query. For each item $j\in L^{\mathcal Q'}$, let $l^{\mathcal Q'}(j)$ be the value of item $j$ for all valuations in $\mathcal V^{\mathcal Q'}$.

We first consider the case where the additional query is a value query, and then the case where the additional query is a demand query. If the algorithm makes a value query for some set $S$, the adversary answers that the value of $S$ is $\epsilon^{\mathcal Q'}\cdot |S\setminus L^{\mathcal Q'}|+\sum_{j\in S\cap L^{\mathcal Q'}} l^{\mathcal Q'}(j)$. This answer is consistent with the previous queries since there exists a valuation $v\in \mathcal V^{\mathcal Q'}$ that obeys the conditions in the statement of the lemma: e.g., $v(\{j\})=l^{\mathcal Q'}$ for every $j\in L^{\mathcal Q'}$ and $v(\{j\})=\epsilon^{\mathcal Q'}$ for every $j\notin L^{\mathcal Q'}$. Define $L^{\mathcal Q}=L^{\mathcal Q'}, \epsilon^{\mathcal Q}=\epsilon^{\mathcal Q'}$ and the set of linear equations $A^{\mathcal Q}$ to be $A^{\mathcal Q'}$ with the additional constraint that $v(S\setminus L^{\mathcal Q'})=\epsilon^{\mathcal Q'} \cdot |S\setminus L^{\mathcal Q'}|$.


%it is consistent with Equation (\ref{eqn-all-epsilon}) as well as with the definition of $L_i$.
%Note that after each such query $t_{i+1}$ has increased by $1$.
%Note that after each such query $t_{i+1}$ and the number of lines in $A_i$ have increased by $1$ and $L_i$ is unchanged.

If the additional query is a demand query, the adversary answers it as follows. Find a sparse solution for the system $A^{\mathcal Q'} \cdot v = \epsilon^{\mathcal Q'}\cdot A^{\mathcal Q'}\cdot \vec{\textbf{1}}$ and $v\geq 0$. 
Since the vector $\epsilon^{\mathcal Q'}\cdot \vec{\textbf{1}}$ is a solution, by Lemma~\ref{lem:sparse} there exists a solution $\vec r\in\R_{+}^{m-|L^{\mathcal Q'}|}$ with at most $t_{i+1}{=t_i+x'}$ non-zero coordinates (recall that $i$ is the number of demand queries in $\mathcal Q'$).
According to Claim~\ref{pro:continuance}, the vector $\vec {r'}=(1-\epsilon^{\mathcal Q}) \vec r+\epsilon^{\mathcal Q}\cdot \vec{\textbf{1}}$ is also a valid solution, for any $\epsilon^{\mathcal Q}$. We choose $\epsilon^{\mathcal Q}$ small enough to ensure that all values which are $0$ in $\vec r$, are still among the $m-|L^{\mathcal{Q}'}|-t_{i+1}$ minimal entries in $\vec r'$.
In addition, $\epsilon^{\mathcal Q}$ is chosen to be strictly smaller than the minimal price of an item in the $(i+1)$'th (last) demand query. 
The adversary then answers the demand query according to the valuation defined by the solution $\vec {r'}$. 

We now show that the induction hypothesis holds for $\mathcal Q$. $\epsilon^{\mathcal Q}$ was already defined. Let $L^{\mathcal Q}$ be $L^{\mathcal Q'}$ with all items that their value is among the highest $t_{i+1}$ values in $\vec r'$. The common value of any such newly added item $j$ in $\mathcal V^{\mathcal Q}$ will be its value in the solution $\vec {r'}$.


%The set of linear equations $A_{i+1,x} $ is obtained from $A_{i,x}$ by then modified to $A_{i+1,x} \cdot  v = \epsilon_{i+1,x}\cdot  A_{i+1,x} \cdot\vec{\textbf{1}}$ by subtracting any item in $L_{i+1,x}$ from both sides of the equation. 
%I.e., every constraint of the form $\sum_{a\in S-L_{i,x}}{v(a)}= b$ is updated to $\sum_{a\in S-L_{i+1,x}}v(a)= b-\sum_{a\in S\cap L_{i+1,x}}v(a)$.


The set of linear equations $A^{\mathcal Q}$ is obtained from $A^{\mathcal Q'}$ by updating every constraint $\sum_{a\in S\setminus L^{\mathcal Q'}}{v(a)}= b$ in $A^{\mathcal Q'}$ to $\sum_{a\in S\setminus L^{\mathcal Q}}v(a)= b-\sum_{a\in S\cap L^{\mathcal Q}}v(a) = \epsilon^{\mathcal{Q}}\cdot |S\setminus L^{\mathcal Q}|$.

Note that $\mathcal V^{\mathcal Q}$ is not empty as it contains the valuation defined by $\vec {r'}$ and the values of the items in $L^{\mathcal Q'}$. Furthermore, all valuations in $\mathcal V^{\mathcal Q}$ are consistent with all queries made so far, and in particular with the last demand query. since all items that are not in $L^{\mathcal Q}$ have values smaller than the minimal price in the last demand query.
%
%We start by defining $L_{i+1,x}$. Since $\epsilon_{i+1,x}$ is smaller than all prices, we have that none of the $m-|L_i|-t_{i+1}$ items of smallest value is in any demand set. Thus the demand query only reveals information on the identity of the $t_{i+1}$ items with the highest values that are not in $L_i$. We conservatively assume that the value of these $t_{i+1}$ items is also known after this query. That is, $L_{i+1} \subseteq L_i\cup\set{x\in\items-L_i|r_x>0}$ and $|L_i|\leq \sum_{j\leq i}{t_j}$.
%In particular, the adversary has not committed on the identity not values of the $m-|L_i|-t_{i+1}$ items with the smallest items (except for the linear constraints implied by the previous queries).
%
%The constraint $A'_{i+1} v = \epsilon_i A'_{i+1} \cdot\vec{\textbf{1}}$ is then modified to $A_{i+1} v = \epsilon_{i+1} A_{i+1} \cdot\vec{\textbf{1}}$ by subtracting any item in $L_{i+1}$ from both sides of the equation. 
%I.e., any constraint of the form $\sum_{a\in S-L_i}{v(a)}= b$ is updated to $\sum_{a\in S-L_{i+1}}v(a)= b-\sum_{a\in S\cap L_{i+1}}v(a)$. 
%Since the new items in $L_{i+1}$ are chosen according to $r'$, we have that the new linear system takes the form $A_{i+1} v = \epsilon_{i+1} A' \cdot\vec{\textbf{1}}$ (i.e., $\sum_{a\in S- L_{i+1}}v(a)=\epsilon_{i+1}|S-L_{i+1}|$) where the dimensions of $A_{i+1}$ are $t_{i+1}\times (m-L_{i+1})$.
%Observe that we modify $A_{i+1}$ to maintain our property with respect to $\epsilon_{i+1}$ without adding new constraints.
%Hence, $t_{i+1}$ is bounded by the number of value queries made so far (independent of the number of non-zero prices demand queries \sd{that does not make sense. any value query can be simulated in our model by one demand query since the demand query also returns the value of the set. maybe it's better to prove this bound only with demand queries?}).\rk{we assumed at beginning of the proof that any query is either a value query or a demand query with no zero prices. This model had the same expressiveness as our original model with same asymptotic sample complexity.}
\end{proof}


Using Claim \ref{claim-invariant} we are now ready to complete the proof of the theorem.
Let $q_v$ be the total number of value queries and $q_d$ be the total number of demand queries made by the algorithm. Let $\mathcal Q$ be the list of queries.
Since the $i$'th demand query adds at most $t_i$ new items to the set $L^{\mathcal Q}$ and $t_i$ is at most $q_v$, the total number of items in $L^{\mathcal Q}$ is $q_v\cdot q_d$. Thus, the linear system has at most $q_v$ constraints. 
Furthermore, each item $j\in L^{\mathcal Q}$ corresponds to a linear constraint of the form $v(j)=t$ for some known value $t$. That is, the set $\mathcal V^{\mathcal Q}$
is non-empty and defined by at most $q_v\cdot q_d+q_v$ linear constraints. When $q_d,q_v \leq \sqrt{m}-1$, we have that the total number of constraints is at most $q_v\cdot q_d+q_v<m-1$. By Lemma~\ref{lem:n_value_queries} the algorithm fails for some valuation $v$.
\comment{
During the run of the algorithm, we maintain two data structures. The first is a set $L$ of items for which the exact value of the item is known. Roughly speaking, we will make sure that every demand query adds not too many items to $L$. The second is a linear system $Av=b$ representing the constraints implied by the answers to the value queries that have been made. %That is, for a query for the value of $S$ we add the equation $\Sigma_{j\in S}v_j=v(S)$.

Let $t_i$ be the number of value queries made before the $i$'th demand query.
The data structures maintain the following inductive property:
after the $i$'th demand query of the algorithm, there exists an $\epsilon_i$ and a matrix $A\in \set{0,1}^{t_i\times (m-|L|)}$, such that all valuations that are consistent with the queries made by this point can be represented as the set $L$ and the following linear system that gives constraints on items that are not in $L$:
\begin{equation}
A\cdot v = \epsilon_i\cdot A\cdot \vec{\textbf{1}}
\end{equation}

We define $\epsilon_0=1$. For every value query made after the $i$'th demand query and before $(i+1)$'th demand query, the adversary answers similarly: $v(S)=\epsilon_i|S- L|+\sum_{j\in S\cap L} v(\{j\})$. This answer is consistent with the previous queries since it is consistent with Equation (\ref{eqn-all-epsilon}) as well as with the definition of $L$.
	
The adversary answers the $(i+1)$'th demand query as follows: find a sparse solution for $Av = \epsilon_i\cdot A\cdot \vec{\textbf{1}}$ and $v\geq 0$. Since the vector that all of its coordinates are $\epsilon_i$ is a solution, Lemma~\ref{lem:sparse} implies that there exists a solution $\vec r\in\R_{+}^{m-|L|}$ with only $t_i$ non-zero coordinates.

According to Claim~\ref{pro:continuance} the vector $\vec {r'}=(1-\epsilon_{i+1}) \vec r+\epsilon_{i+1}\cdot \vec{\textbf{1}}$ is also a valid solution for any $\epsilon_{i+1}$. We choose $\epsilon_{i+1}$ small enough to ensure that %for any pair of items $i,j$ we have that $r'_i>r'_j$ if and only if $r_i>r_j$ \sd{"X if and only if X" is not a very interesting statement}. That is, 
all values which are $0$ in $\vec r$, are still among the $m-|L|-t_i$ minimal entries in $r'$ \sd{do you mean $m-\sum_it_i?$}. \rk{yes. maybe clearer: among the $m-|L|-t_i?$}
In addition, $\epsilon_{i+1}$ is chosen to be strictly smaller than the minimal price of an item at the $(i+1)$'th demand query. 

The adversary then answers the demand query according to the solution $\vec {r'}$. Since $\epsilon_{i+1}$ is smaller than all prices, we have that none of the $m-|L|-t_i$ items of smallest value are in any demand set. Thus the demand query only reveals the identity of the $t_i$ items with the highest values that are not in $L$. We conservatively assume that the value of these $t_i$ items is also known after this query.
%That is the information revealed by the $i$-th demand query is no more than getting the exact values of the top $t_i$ values.
%We assume that after this query, all top $t_i$ values are revealed and are now in the $L$ of known values.
%by returning the value of each of the $t_i$ items of value larger than $\epsilon_{i+1}$ (and they are added to $L$). 
%Since only other items are guaranteed to be in demand, committing to the value of those is sufficient information to answer the demand query \sd{what???}, this is sufficient information \sd{sufficient for what?}.
%\footnote{The assumption that all top $t_i$ values are revealed and not just their sum reveals more information than in the standard query model. As we show now, the $\sqrt{n}$ lower bound still holds with this additional information. }%However, in this model there is an algorithm that reaches that lower bound which is not implantable in the standard model.}
%\sd{this is not clear}
%In general, demand queries do not reveal the value of each returned item separately but rather their sum. As we now show, the lower bound holds with this additional information.} 
In particular, the adversary has not committed on the identity not values of the $m-|L|-t_i$ items with the smallest items (except for the linear constraints implied by the previous queries).

We then modify the constraint $A v = \epsilon_i A \cdot\vec{\textbf{1}}$ by subtracting any new item in $L$ from both sides of the equation. 
I.e., any constraint of the form $\sum_{a\in S}= b$ is updated to $\sum_{a\in S-L}v(a)= b-\sum_{a\in S\cap L}v(a)$. 
Since the new items in $L$ are chosen according to $r'$, we have that the new linear system takes the form $A' v = \epsilon_{i+1} A' \cdot\vec{\textbf{1}}$ (i.e., $b-\sum_{a\in S\cap L}v(a)=\epsilon_{i+1}|S-L|$) where the dimensions of $A'$ and $A$ are the same.
Observe that we modify $A$ to maintain our property with respect to $\epsilon_{i+1}$ without adding new constraints.
Hence, $t_i$ is bounded by the number of value queries made so far (independent of the number of demand queries \sd{that does not make sense. any value query can be simulated in our model by one demand query since the demand query also returns the value of the set. maybe it's better to prove this bound only with demand queries?}).\rk{we assumed at beginning of the proof that any query is either a value query or a demand query with no zero prices. This model had the same expressiveness as our original model with same asymptotic sample complexity.}

Let $q_v$ be the total number of value queries and $q_d$ be the total number of demand queries made throughout the algorithm.
Since the $i$'th demand query adds at most $t_i$ new items to the set $L$ and $t_i$ is at most $q_v$, the total number of items in $L$ at the end of the algorithm is $q_vq_d$ and the linear system has at most $q_v$ constraints. 
At the end of the algorithm, Each item in $x\in L$ corresponds to a linear constraint of the form $v(x)=t$ for some known value $t$. That is, the two data structures are translated to a set of at most $q_vq_d+q_v$ constraints.
By making at most $\sqrt{m}-1$ queries of each type, we have that the total number of constraints is at most $q_vq_d+q_v<m-1$. By Lemma~\ref{lem:n_value_queries} the algorithm fails for some valuation $v$.
}
\end{proof}

%\sd{
%	The additive setting has some interesting connections to some classic problems. One is the selection problem ($https://en.wikipedia.org/wiki/Selection_algorithm$) where the goal is to return the $k$th highest number. The other is unordered partial sorting (in the same link) in which the goal is to find the highest $k$ numbers (unordered). Note that the selection problem can be solved by running two calls to an algorithm for unordered partial sorting (one with a parameter of $k$ and the other with parameter $k-1$).
%	
%	Unordered partial sorting can be solved in $\O{m\log m}$ time by quickselect which is a variant of quicksort. Quickselect is simply our algorithm for the distinct values case, where the pivot procedure of quicksort is implemented by a uniform-price demand query. Indeed, quickselect makes $O{\log m}$ pivot calls, each takes $\O{m}$ time. (When items are not distinct things are more complicated for us because we do not have control on the implementation of the pivot procedure). 
	
%	There are some lower bounds on the number of queries for selection\\ (jeffe.cs.illinois.edu/teaching/497/02-selection.pdf) but as far as I can tell they work on the comparison model, just like the lower bounds on sorting that you learn in algorithms course. In that light, we explore the complexity of pivot-based algorithms. Our lower bound shows that randomization is essential to quickselect and other pivot-based algorithms in the sense that we need $\Om{\sqrt{m}}$ pivot and value queries. Note that there are algorithm like Introselect\\ (https://en.wikipedia.org/wiki/Introselect) that use the median of the medians algorithm to deterministically ensure a good selection of the pivot for quickselect. However, these algorithms use many value queries, and our lower bound shows that this is unavoidable.
%}



==> old/model_old.tex <==
\section{Model and Preliminaries}\label{sec:model}
\paragraph{Valuations.}
A valuation is a function $v:2^\items\rightarrow\R_{+}$ where we denote $\items = \set{1,\ldots, m}$ as the set of {\em items} and $v(S)$ is the {\em value} of a bundle $S\subseteq \items$.
We denote by $v(T|S) = v(S\cup T)-v(S)$ the marginal contribution of set $T$ to set $S$. 
We abuse notation and use $f(a)$ and $f(a|S)$ to denote $f(\set{a})$ and $f(\set{a}|S)$, for $a\in \items$.
We list here the classes of valuations discussed in this work. 

\begin{itemize}
	 
	\item A valuation $v$ is \emph{additive} function if for all $S\subseteq \items$ we have that $v(S)=\sum_{a\in S}v(\set{a})$.
	\item A valuation $v$ is \emph{budget-additive} function if there exist a budget $b\in\R$ such that for all $S\subseteq \items$ we have that $v(S)=\min\set{b,\sum_{a\in S}v(\set{a})}$. \rk{relevant?}
	\item A valuation $v$ is \emph{submodular} function if it exhibits the diminishing returns property, i.e., $f(a|S)\geq f(a|T)$ for all    $S\subseteq T \subseteq \items$ and  $a\in \items$.
	\item A valuation $v$ is a \emph{coverage} function if there exists a universe $U$ with non-negative weights $w(u)$ for each $u\in U$ and subsets $A_1, A_2,\ldots, A_n$ of $U$ such that $v(S) = \sum_{u\in \bigcup_{i\in S} A_i}w(u)$.
%, where $f_{S}(T):=f(S\cup T)-f(S)$ is the marginal contribution of  $T$ to  $S$. We abuse notation and write $f(a)$, $f_S(a)$ for $f(\{a\})$ and $f_S(\{a\})$ when clear from context.
	\item A valuation $v$ is \emph{sub-additive} function if for all $S\subseteq \items$ we have that $v(S)\leq\sum_{a\in S}v(a)$.
	\item A valuation $v$ is a \emph{gross substitutes} function if it is submodular and for any $S,T$ and for every $s\in S$ we have that at least one of the following must hold: 
	\begin{enumerate}
		\item $v(S)+v(T)\leq v(S\setminus\set{s})+v(T\cup\set{s})$
		\item There exists an item $t\in T$ such that $ u(S)+u(T)\leq u(S\setminus\set{s}\cup\set{t})+u(T\setminus \set{t}\cup \set{t})$
	\end{enumerate}
	There are many other equivalent definitions for gross substitutes, see \cite{leme2017gross} for a survey.
	\item A valuation $v$ is \emph{unit-demand} function if for all $S\subseteq \items$ we have that $v(S) = \max_{a\in S}v(a)$. \rk{relevant?}
\end{itemize}
When $v$ is an additive valuation we represent the function as a vector $v = (v_1,...,v_m)\in \R^m$, where $v_i\geq 0$ is the value of the $i$-th item.

We have that $additive\subset gross~substitutes\subset submodular$ (see  \cite{LehmannLehmannNisan}).
%The relations between the classes is demonstrated in Figure~\ref{fig:classes}.

\paragraph{Maximization Under Cardinality Constraint}
Given a valuation $v$ over set $\items$, we wish to find a set that maximize the function under a constraint $\mathcal{S}\subseteq 2^\items$, i.e., to find $$\OPT \in \arg\max_{S\in\mathcal{S}}(v(S)).$$
%We say that a set $S$ is $\alpha$ approximation to the optimal solution if $S\in\mathcal{M}$ and $f(S)\geq \alpha\OPT$.
In most of the work we focus on cardinality constraints, i.e., $\mathcal{S} = \binom{\items}{k}$ for some known parameter $k$ and denote this problem {\em finding an optimal set of size $k$}. \rk{better naming? $\OPTK$?}

\paragraph{Menu.}
Given a set $\items$ of $m$ items, a {\em menu} is a set of pairs $\set{\Delta_i ,p_i}$, where $\Delta_i$ is a distribution over subsets of items and $p_i$ is the price to participate in a lottery which gives the buyer a random set sampled from $\Delta_i$.
In this work we consider only deterministic menus, i.e., all menu entries offer bundles and not a lotteries over bundles.
Given a set $\items$ of $m$ items, a {\em deterministic menu} is a set of pairs $\set{S,p_S}$ of bundles and prices. \footnote{We assume free disposal of items by the buyer, i.e., for any $S,T\subseteq \items$ such that $S\subseteq T$ we have that $p_S\leq p_T$ (otherwise $S$ is never being sold) and that the menu includes the option of receiving the empty set for free.} 
Given a valuation $v$, a buyer selects a bundle $S$ that maximizes her utility, i.e. $\arg\max_{S'\subseteq \items}v(S')-p_S$.  
A seller who has only ex-ante information on $v$, i.e., knows the distribution $\mathcal{F}$ from which $v$ is drawn, wishes to present a menu that maximizes her expected revenue.



\begin{itemize}
	\item $\REV_{\menu}(v)$ - the revenue of the seller from menu $\menu$ when the buyer's valuation is $v$, i.e., the price of the menu entry chosen by the buyer. 
	\item $\REV(\menu,\mathcal{F})$ - the expected revenue where the expectation is over the buyer's valuation $v\sim\mathcal{F}$.
	\item $\REV(\mathcal{F})$ - The optimal revenue obtained by any possible menu when the buyer profile is drawn from $\mathcal{F}$.
	\item $\DREV(\mathcal{F})$ - The optimal revenue obtained by any deterministic menu when the buyer profile is drawn from $\mathcal{F}$.
	\item $\SREV(\mathcal{F})$ - The optimal revenue obtained by selling each item separately for its own Myerson's optimal take-it-or-leave-it price \cite{myerson1981optimal}, when the buyer profile is drawn from $\mathcal{F}$.
	\item $\BREV(\mathcal{F})$ - The optimal revenue obtained by selling all items as a single bundle for its Myerson’s optimal price, when the buyer profile is drawn from $\mathcal{F}$.
	\item $\SYMREV(\mathcal{F})$ - The optimal revenue obtained by a menu who is indifferent regarding the items' names, when the buyer profile is drawn from $\mathcal{F}$.
	\item $\SYMDREV(\mathcal{F})$ - The optimal revenue obtained by a deterministic menu mechanism who is indifferent regarding the items' names, when the buyer profile is drawn from $\mathcal{F}$. I.e., a menu that prices a bundle solely according to its size.
\end{itemize}

In addition, we denote by $H_{\menu}$ the ratio between the maximal and minimal non-zero prices in a given menu $\menu$. For integer prices this is simply the maximal price in the menu. When clear from context we omit $\menu$ and use $H$. \rk{maybe to define only in the relevant section}

\paragraph{Symmetric deterministic menu.} A symmetric deterministic menu can be represented as a set of offers $(q_i,p_i)$ of the form ``pay $p_i$ and choose any set of size $q_i$ of items to receive". Since a buyer can dispose items, we assume that all $q_i>q_j$, we have that $p_i>p_j$ (all inequalities are strict).
%We refer to the number of different bundle sizes offered as the number of {\em levels} a symmetric menu has.
(we omit "deterministic" when clear from context)

\paragraph{Queries.}
Given a valuation $v$ over set $\items$ of size $m$, we consider two common ways to access the values of $v$ (which may have an exponential representation): value and demand queries.
A {\em value query} on $S$ simply asks for the value of a bundle $v(S)$.
A {\em demand query} asks for a bundle of maximal utility (i.e., a set in demand) given a price vector $\textbf{p} = (p_1,\cdots,p_m)\in \R^{m}_{+}$. Formally, $D(\textbf{p}) \in \arg\max_{S\subseteq \items}{\left(v(S)-p(S)\right)}$ where $p(S)=\sum_{i\in S}p_i$, if there are several sets in demand one of them is chosen arbitrarily. In this work we assume that the value $\max_{S\subseteq \items}{\left(v(S)-p(S)\right)}$ is also returned as part of the query. \footnote{Hence, any value query $S$ can be implemented using a demand query asking zero prices items in $S$ and infinity prices for any other item}. 
When all the coordinates of $\textbf{p}$ have the same value $p$, we refer to the corresponding query as a {\em uniform demand} query for price $p$.
\rk{to mention linear queries here? only relevant for additive valuations and for a very small part of our work}

\paragraph{Query complexity.\rk{Oracle complexity?}}
The query complexity of a valuation $v$ in menu $\menu$ under algorithm $\ALG$ is the number of queries made by an algorithm $\ALG$ looking for a profit-maximizing menu entry for $v$ in menu $\menu$.

We say that an algorithm has a {\em query complexity} $T$ if the expected number of queries asked by the algorithm is at most $T$, where the expectation is taken only over random decisions made by the algorithm and the worst-case of an input $v$. I.e., this is a bound on the expected number of queries for any possible input. 

We say that an algorithm has a {\em distributional query complexity} $T$ over valuation distribution $\mathcal{F}$ if the expected number queries asked by the algorithm is $T$ where the expectation is over the valuation input $v\sim\mathcal{F}$ and possibly random decisions made by the algorithm. 

The queries we are counting are either value or demand queries and the algorithm can be either deterministic or randomized one.
That is, we consider 8 different complexity measures $\set{\text{deterministic, randomized}}\times\set{\text{value queries, demand queries}}\times\set{\text{worst-case, distributional}}$.
Most of the work is under the randomized demand queries worst-case query complexity measure and we use the notion {\em query complexity} for this measure when clear from context.




\mbc{==========================================\\ OLD stuff from here to the end of the section, to be removed after the above is approved:}

\paragraph{Menu. }
The above optimization problem is tightly  related to the problem of implementing an auction between a buyer with a valuation $v$ over a set of items and the seller who possesses those items. When having a single pair of a seller and a buyer, any auction can be represented as a menu.

Given a set $\items$ of $m$ items, a {\em menu} is a set of pairs $\set{\Delta_i ,p_i}$, where $\Delta_i$ is a distribution over subsets of items and $p_i$ is the price to participate in a lottery which gives the buyer a random set sampled from $\Delta_i$.
In this work we consider only deterministic menus, i.e., all menu entries offer bundles and not lotteries over bundles.
Given a set $\items$ of $m$ items, a {\em deterministic menu} is a set of pairs $\set{S,p_S}$ of bundles and prices. \footnote{We assume free disposal of items by the buyer, i.e., for any $S,T\subseteq \items$ such that $S\subseteq T$ we have that $p_S\leq p_T$ (otherwise $S$ is never being sold) and that the menu includes the option of receiving the empty set for free.} 
Given a valuation $v$, a buyer selects a bundle $S$ that maximizes her utility, i.e. a set in $\arg\max_{S'\subseteq \items}v(S')-p_{S'}$.  
A seller who has only ex-ante information on $v$, i.e., knows the distribution $\mathcal{F}$ from which $v$ is drawn, wishes to present a menu that maximizes her expected revenue.

In this work, we focus on a family of menus that only care about the amount of sold items and do not distinguish between different items.
A {\em symmetric deterministic menu} is a set of offers $(q_i,p_i)$ of the form ``pay $p_i$ and choose any set of size $q_i$ of items to receive". Since a buyer can dispose items, we assume that all $q_i>q_j$, we have that $p_i>p_j$ (all inequalities are strict).
%We refer to the number of different bundle sizes offered as the number of {\em levels} a symmetric menu has.
%(we omit "deterministic" when clear from context)
The connection to \opt{k} sets is intuitively obvious and is shown formally in this work.

A key characteristic of a menu is the amount of revenue expected for a seller who uses this menu. We define the following notation regarding the revenue extracted from menus. 
\begin{itemize}
	\item $\REV_{\menu}(v)$ - the revenue of the seller from menu $\menu$ when the buyer's valuation is $v$, i.e., the price of the menu entry chosen by the buyer. 
	\item $\REV(\menu,\mathcal{F})$ - the expected revenue where the expectation is over the buyer's valuation $v\sim\mathcal{F}$.
%	\item $\REV(\mathcal{F})$ - The optimal revenue obtained by any possible menu when the buyer profile is drawn from $\mathcal{F}$.
%	\item $\DREV(\mathcal{F})$ - The optimal revenue obtained by any deterministic menu when the buyer profile is drawn from $\mathcal{F}$.
%	\item $\SREV(\mathcal{F})$ - The optimal revenue obtained by selling each item separately for its own Myerson's optimal take-it-or-leave-it price \cite{myerson1981optimal}, when the buyer profile is drawn from $\mathcal{F}$.
%	\item $\BREV(\mathcal{F})$ - The optimal revenue obtained by selling all items as a single bundle for its Myerson’s optimal price, when the buyer profile is drawn from $\mathcal{F}$.
%	\item $\SYMREV(\mathcal{F})$ - The optimal revenue obtained by a menu who is indifferent regarding the items' names, when the buyer profile is drawn from $\mathcal{F}$.
	\item $\SYMDREV(\mathcal{F})$ - The optimal revenue obtained by a deterministic menu mechanism that is indifferent regarding the items' names, when the buyer profile is drawn from $\mathcal{F}$. I.e., a menu that prices a bundle solely according to its size.
	\item \rk{Removed: \REV,\DREV,\SREV,\BREV,\SYMREV}
\end{itemize}


%In addition, we denote by $H_{\menu}$ the ratio between the maximal and minimal non-zero prices in a given menu $\menu$. For integer prices this is simply the maximal price in the menu. When clear from context we omit $\menu$ and use $H$. \rk{maybe to define only in the relevant section}

\paragraph{Queries.}
\rk{Even the very simple menu that sells each item separately for the same fixed price $p$ has an exponential number of menu entries, as it should have an entry for every one of the $2^m$ bundles. This motivates the exploration of other representation schemes that capture simplicity in a refined way.}

Given a valuation $v$, we consider two ways to access the values of $v$ (which may have an exponential representation): value queries and demand queries.
A {\em value query} of a set $S$ simply asks for the value of the bundle $v(S)$.
A {\em demand query} asks for a bundle of maximal utility  at some given item prices, i.e., a set in demand, given a price vector $p = (p_1,\cdots,p_m)\in \R^{m}_{+}$. Formally, the query returns an arbitrary set $D \in \arg\max_{S\subseteq \items}{\left(v(S)-p(S)\right)}$ where $p(S)=\sum_{i\in S}p_i$. The fact that the returned set might might be chosen in the worst way for our algorithm is a main concern in this work, and this is the assumption taken throughout the paper. In this work we assume that the value $\max_{S\subseteq \items}{\left(v(S)-p(S)\right)}$ is also returned as part of the query. \footnote{Hence, any value query $S$ can be implemented using a demand query asking zero prices items in $S$ and infinity prices for any other item}
When all the coordinates of $p$ have the same value $t\in\R$, we refer to the corresponding query as a {\em uniform demand} query for price $t$.
\rk{Removed: linear queries. Only relevant in a very small part of our work}

\paragraph{Query complexity.\rk{Oracle complexity?}}
The query complexity of a valuation $v$ under some algorithm $\ALG$ is the number of queries made by the algorithm.

We say that an algorithm has a {\em query complexity} $q$ if the expected number of queries asked by the algorithm is at most $q$, where the expectation is taken only over random decisions made by the algorithm and the worst-case of an input $v$. I.e., this is a bound on the expected number of queries for any possible input. 

We say that an algorithm has a {\em distributional query complexity} $q$ over a distribution $\mathcal{F}$ if the expected number queries asked by the algorithm is $q$ where the expectation is over the valuation input $v\sim\mathcal{F}$ and possibly random decisions made by the algorithm. 

The queries we are counting are either value or demand queries and the algorithm can be either deterministic or randomized.
That is, we consider 8 different complexity measures $\set{\text{deterministic, randomized}}\times\set{\text{value queries, demand queries}}\times\set{\text{worst-case, distributional}}$.
Most of the work is under the randomized demand queries worst-case query complexity measure and we use the notion {\em query complexity} for this measure when clear from the context.

The algorithms discussed in this work are either for finding a \opt{k} set or for implementing a menu. We say that a menu $\menu$ has a query complexity $q$ (in any of the above models) if there exists an algorithm that implements this menu and has a query complexity $q$.










--------------- old all equal t for additive proof-


	\mbc{==========================\\ OLD FROM HERE (should be removed after the above is approved) :\\}
Let $H = \set{v>t\mid v\in S}$ be the unknown set of items in $S$ with values strictly larger than $t$. We can check whether or not $H$ is empty, by making a single value query of the entire set $S$.	If it is the case that $v(S) = t\cdot|S|$, the algorithm terminates since all the items in $S$ are of value $t$.	Else, $v(S)>t\cdot|S|$, and we use the following version of binary search to sample a random item $v\in H$ and after doing so, updating $S$ according to the new information.	We split $S$ randomly into two sets $S_0,~S_1$ such that $||S_0|-|S_1||\leq 1$.	For each one of the sets, we test if it contains at least one item with a value higher than $t$ by querying for the total value of the set as before.	For at least one of the sets, the answer must be positive and we continue with this set. If both answers are positive, we choose one of them at random. We continue splitting randomly until we remain with a single item of value $v>t$ that is chosen randomly from $H$. This process is done using $\O{\log m}$ value queries. 
	
\mbc{OLD:}	Thus, by making a uniform demand query with the price $\frac{v+t}{2}$ for each item in $S$, and keeping in $S$ only items from $S$ who are \textbf{not} in the demand, we eliminate in expectation at least half of $L$ as being items of value $t$  while keeping all of the items of price exactly $t$.
	Thus, $\O{\log m}$ rounds with $\O{\log m}$ value queries and a single demand query, suffice in expectation in order of identifying all occurrences of value $t$ in $D$.
	
\mbc{OLD:}	The set $C$ is handled in the exact same way, but now we update $S$ to include items that are \textbf{in} the demand for uniform price $\frac{v+t}{2}$ for $v$ sampled from $H = \set{v<t\mid v\in S}$ as before.



=================
In this paper we revisit the notion of simplicity in mechanisms. We consider a seller of $m$ heterogeneous items, facing a single buyer with valuation $v$. We observe that previous attempts to define complexity measures often fail to classify mechanisms that are intuitively considered simple (as ``selling separately''), as such. We suggest to view a menu as simple if a bundle that maximizes the buyer's profit can be found by conducting a few primitive operations that are considered simple. The primitive operation that we consider in this paper is essentially running the common ``selling separately'' auction, and we measure complexity in terms of the number of primitive operations needed to (adaptively) find a profit-maximizing entry in the menu. We call this measure the \emph{primitive complexity of a menu}.
We connect the notion of primitive complexity  to the vast literature on the query complexity of various tasks in different valuations classes. 

Does the primitive complexity  capture the simplicity of other auctions that are intuitively simple? We consider \emph{bundle-size pricing},  a common pricing method in which the price of a bundle depends only on its size.
Our main technical contribution is determining the primitive complexity  of various bundle-size pricing menus. 
We show that for any distribution $\D$ over weighted matroid rank valuations, even distributions with arbitrary correlation among their values, there is always a bundle-size pricing menu with low primitive complexity  that achieves almost the same revenue as the optimal bundle-size pricing menu. As part of this proof we provide a randomized algorithm that for any weighted matroid rank valuation $v$ and integer $k$, finds the most valuable set of size $k$ with only a poly-logarithmic number of demand and value queries. We show that this result is essentially tight in several aspects. For example, if the valuation $v$ is submodular, then finding the most valuable set of size $k$ requires exponentially many queries (this solves an open question of Badanidiyuru et al. [EC'12]). We also show that any deterministic algorithm that finds the most valuable set of size $k$ requires $\Omega(\sqrt m)$ demand and value queries, even for additive valuations.








In this paper we revisit the notion of simplicity in mechanisms. We consider a seller of $m$ heterogeneous items, facing a single buyer with valuation $v$. We observe that previous attempts to define complexity measures often fail to classify mechanisms that are intuitively considered simple (e.g., the ``selling separately'' mechanism) as such. We suggest to view a menu as simple if a bundle that maximizes the buyer's profit 	can be found by conducting a few primitive operations that are considered simple.  
The \emph{primitive complexity of a menu} is the number of primitive operations needed to (adaptively) find a profit-maximizing entry in the menu.  In this paper, the primitive operation that we study is essentially computing the outcome of the ``selling separately'' mechanism. 
		
Does the primitive complexity  capture the simplicity of other auctions that are intuitively simple? We consider \emph{bundle-size pricing},  a common pricing method in which the price of a bundle depends only on its size.
Our main technical contribution is determining the primitive complexity of bundle-size pricing menus in various settings. First, we connect the notion of primitive complexity  to the vast literature on query complexity. We then show that for any distribution $\D$ over weighted matroid rank valuations, even distributions with arbitrary correlation among their values, there is always a bundle-size pricing menu with low primitive complexity  that achieves almost the same revenue as the optimal bundle-size pricing menu. As part of this proof we provide a randomized algorithm that for any weighted matroid rank valuation $v$ and integer $k$, finds the most valuable set of size $k$ with only a poly-logarithmic number of demand and value queries. We show that this result is essentially tight in several aspects. For example, if the valuation $v$ is submodular, then finding the most valuable set of size $k$ requires exponentially many queries (this solves an open question of Badanidiyuru et al. [EC'12]). We also show that any deterministic algorithm that finds the most valuable set of size $k$ requires $\Omega(\sqrt m)$ demand and value queries, even for additive valuations.


==> oneitem.tex <==
\section{Finding an item of maximal value}\label{sec:oneitem}
\rk{TODO: split results between upper and lower sections and remove this one}

In this section we focus on the problem of finding a single item of maximal value, i.e., cardinality constraint of $k=1$.
Note that this problem can be solved deterministically using $n$ singleton value queries for any valuation. We first show that using randomized demand queries,  a polylogarithmic number of queries suffices for solving this problem.

\begin{proposition}%\label{thm:findmaxSA}
	Given a \textbf{sub-additive} valuation $v:2^N\rightarrow\R$, there exists a randomized algorithm, with $\O{\log^2 n}$ \textbf{demand} query complexity, that finds a \textbf{single item} of maximal value.
\end{proposition}
\rk{proof moved to upper bound section}




On the other hand, finding a set maximal set of size larger than one requires much more demand queries even for $k=2$ and the class of submodular valuations, and we elaborate on this in Section~\ref{sec:lb}.

%As shown in Section~\ref{sec:algorithms}, for any sub-additive valuation, we can find a maximal (single) item using polylog(n) many queries.
Randomization is indeed necessary: In Section~\ref{sec:lb} we show that for additive valuations, any deterministic algorithm that finds an item of minimal value requires at least $\sqrt{n}$ demand queries. Here we show a simple reduction that shows that for additive valuation this is essentially the same problem as finding an item of maximal value.

\begin{lemma}
	minimum and maximum are the same
\end{lemma}
\begin{proof}
	Let $H = v(N)$ be a bound on the maximal value of any item. Any maximal finding algorithm can be reduced to vvvvvvvvvvvvv.
	For each value query $S$ we ask for the value on the original valuation and return $H|S|-v(S)$.
	For each demand query $p$ we ask for the demand for price $H\textbf{1}-p$ on the original valuation and return the completing set.
	
\end{proof}

\paragraph{randomized, communication complexity argument even for $k=1$.}

\rk{communication lower bound for valuations? here or in the lower bound section? Thm: additive valuation, randomized-value-query algorithm, finding maximal item requires n/logn}

We prove our lower bound using a reduction to the Set Disjointness (DISJ) communication problem.
In this problem, two parties, Alice and Bob, are given with two input vectors $x=(x_1,...,x_n),~y=(y_1,...yx_n)\in\set{0,1}^n$ respectively, and they wish to compute the function $f(x,y)$ which defined as: $f(x,y)=1$ if there exists an index $i$ such that $x_i=y_i=1$ and $f(x,y)=0$ otherwise.
It is known that the randomized communication complexity of DISJ is $\Om{n}$, see, e.g., \cite{razborov1990distributional}.\\
Assume in contradiction that there exists an algorithm that for any additive valuation finds the maximal entry using less than $n/\log n$ value queries.

\begin{lemma}
	Given an additive valuation over $n$ items, any algorithm that finds a maximal item with constant probability using only value queries, must mage $\Om{n/\log n}$ queries.
\end{lemma}
\begin{proof}
We build the following reduction:
Given an input $x,y\in\set{0,1}^n$ for the disjointness problem, we define $v\in \set{0,1,2}^n$ to be their sum $v = x+y$.
Assuming there is value querying algorithm for finding maximal entry in $v$, we build the next protocol for DISJ.
For each query $S$, both Alice and Bob each compute the total number of 1 entries in the relevant indexes corresponds to $S$ in their inputs and send it using $\log n$ bits. The fact that $v(S) = x(S)+y(S)$ allows both sides to compute $v(S)$ using a logarithmic number of communication bits. By induction, they can now continue and follow the querying algorithm.
The maximal value in $v$ equals $2$ if and only if there exists an index who is $1$ for both Alice and Bob. Thus, if we were able to find the maximal value using $o(n/\log n)$ value queries, we could have solved DISJ using $o(n)$ communication bits. 
\end{proof}

\rk{example for finding 1-optimal set for general valuation moved so appendix}

==> related.tex <==
\subsection{Related Work}\label{sec:related}
\citet{blumrosen2010computational}
\citet{badanidiyuru2012optimization}

\paragraph{Optimal menus.}
\paragraph{Symmetric menus.} 
\paragraph{Menu complexity.} (including multi choice menus)
\paragraph{Optimization using demand queries.}
\paragraph{Optimization using value queries.} (including linear queries)


==> results.tex <==
\subsection{Results}\label{sec:results}

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{classes}
	\caption{Relations between the subclasses in this work. UD's oracle complexity is constant, all other green classes have a polylogn oracle complexity, coverage has at least linear, SM is exponential}
	\label{fig:classes}
\end{figure}

\subsubsection{menus}
Symmetric menus using demand queries

\begin{theorem}
	Given a symmetric menu $M_1$, there exists a (symmetric) menu $M_2$ such that for any gross substitutes or budget additive valuation $v$, $Rev_{M_2}(v)\geq(1-\epsilon)Rev_{M_1}(v)$ and $M_2$'s expected query complexity (for all additive $v$) is $\O{\log^2 n\cdot \log H_{M_1}}$ where the expectation is over the internal random coins of the algorithm.
\end{theorem}

\begin{theorem}
	Given a distribution over any gross substitutes or budget additive \rk{can be mixed?} valuations $\mathcal{F}$, and a deterministic symmetric menu $M_1$, there exists a (symmetric) menu $M_2$ such that $\mathbb{E}_{v\sim\mathcal{F}}[Rev_{M_2}(v)]\geq(1-\epsilon)\mathbb{E}_{v\sim\mathcal{F}}[Rev_{M_1}(v)]$ and $M_2$ expected (over $\mathcal{F}$) query complexity is $polylog n$ where the expectation is over the internal random coins of the algorithm and the distribution $\mathcal{F}$. 
	%for GS as well????
\end{theorem}

There are complex menus for additive valuations (selling $m/4$ succeeding pairs)

\subsubsection{maximizing under cardinality constraint}
\rk{result list from doc\\expectation vs. h.p.}

\paragraph{Finding maximal item.} For the case of finding a single item of maximal value, i.e., the cardinality constraint  $k=1$, we show an algorithm that works for any \textbf{sub-additive} valuation and makes polylogarithmic many demand queries in expectation. We complete this results with the following lower bounds:
\begin{itemize}
	\item For general (even monotone) valuations, $\Omega(n)$ demand queries are needed in order of finding a single item of maximal value with non negligible probability .
	\item Using only value queries, even for additive valuations, any algorithm that finds a single item of maximal value has a randomized query complexity of at least $n/log n$.
\end{itemize}

\paragraph{General cardinality constraint - algorithmic results.}
Given a gross-substitutes valuation over $n$ items, there exists a randomized algorithm that finds the $k$ items with the highest value and has a query complexity of order $polylog n$ in expectation.
We also show it for additive (warm-up) and budget additive.

\paragraph{General cardinality constraint - lower bounds.}  
GS is best we can hope for - Given a submodular valuation, any algorithm that finds the $k$ items of highest value has an exponential query complexity. (warm-up with coverage functions)

Randomization is crucial - Any deterministic algorithm that finds the $k$ items of highest value (even for additive valuations, k=n-1) has a query complexity of $\Omega(\sqrt{n})$.

Demand queries are crucial - Given an additive valuation, any algorithm that finds the $k$ items of highest value using only value queries has a deterministic query complexity of $n-1$. Any randomized has a query complexity of at least $n/log n$ (we show this for $k=1$ using a communication complexity technique, here we give a different proof using information arguments).


==> symmetricmenumotivation.tex <==
\section{Symmetric menus are interesting \sd{Remove this section}}
We start examples demonstrating the advantage of general symmetric menus compared to the benchmarks of selling each item separately and the menu that only offers a take-it-or-leave-it offer over the grand bundle of items. 

\paragraph{Constant gap between $\SymDREV$ to $\max\{\SREV,\BREV\}$ for i.i.d. additive valuations even when $n$ grows.}
We show that even for valuations drawn from an i.i.d. distribution (where it is known that $\max\{\SREV,\BREV\}$ gives a constant approximation for the optimal revenue \cite{babaioff2014simple}), the difference between $\max\{\SREV,\BREV\}$ and the optimal symmetric menu bounded away from $1$.

A known example where both selling separately and in a bundle fail to gain the maximal revenue is when $v_1,v_2\sim \{0,1,2\}$ with probability $\frac{1}{3}$ for each value.
In this case, the optimal menu offers any single item for $2$ and the grand bundle for $3$, resulting a revenue of $\frac{13}{9}$, which is larger than the revenue of $\frac{12}{9}$ obtained either from selling the two goods separately or from selling them as a single bundle.
One would suspect that as number of items grows, we might be able to use the fact that the distributions are independent and identical and thus using standard concentration lemmas, could show that this gap vanishes. Unfortunately, this is not true, and we extend the above result by showing that for any $n$ there is a \textbf{bounded} i.i.d. distribution $\mathcal{D}_n$ such that $\SymDREV/\max\{\SREV,\BREV\}>1.1$.

$$v_i = \begin{cases}
0& \text{with probability }1-\frac{1}{n}\\
1& \text{with probability }\frac{1}{2n}\\
2& \text{with probability }\frac{1}{2n}\\
\end{cases}$$
$\max\{\SREV,\BREV\} = 1$ while  $\SymDREV>1.1$ by selling any two (or less) items for $2$ and any three (or more) items for $3$.


\paragraph{Gap between $\SymDREV$ to $\max\{\SREV,\BREV\}$ for correlated symmetric items is unbounded.}
As mentioned, for i.i.d variables it is known that  $\max\{\SREV,\BREV\}$ is a constant approximation for $REV$, and hence for $DREV$ as well.
For correlated identically distributed variables, it is known that  $\max\{\SREV,\BREV\}$ fails to achieve any approximation for $REV$ \rk{HartNisan12? is it that "known"?}.
We strength this result and show that  $\max\{\SREV,\BREV\}$ fails to achieve any approximation even when compared to $DREV$.

Consider the following correlated distribution $\mathcal{D}$ over additive valuations over $n$ items.
Let $A_d$ the following set of valuations:
we choose uniformly at random a permutation $\sigma\in \mathcal{S}_n$. In addition, we choose an index $d\in [n]$ randomly such that $\Pr(d\geq j)=\frac{1}{2j^2}$ for $j=2\ldots n$ and $\Pr(d\geq 1)=1$.
We then have that
$$v_i = \begin{cases} d &\mbox{if } \sigma(i) \leq d \\
0 & \mbox{otherwize}\end{cases}.
$$
That is, we choose $d$ random items to have a value $d$ each and the rest of the items are worth $0$, this is done with some distribution over $d$. This is trivially a symmetric distribution.
\begin{theorem}
	$\SymDREV(\mathcal{D}) > \frac{\ln(n)}{2}\cdot\max\{\SREV,\BREV\}$.
\end{theorem}
\begin{proof}
	First we fine the optimal selling-separately mechanism. This is done by computing for each item $\max_p\set{p\cdot \Pr(v_i\geq p)}$ which is maximized for $p=1$ with expected revenue of $1/n$ for any item and revenue of $1$ in total.

	For the optimal selling-grand-bundle mechanism, we compute $\max_p\set{p\cdot \Pr(\sum{v_i}\geq p)}$ which is maximized for $p=1$ with an expected revenue of $1$ (with probability $1$).

	However, the following deterministic menu has an expected revenue which is unbounded.
	The seller offers any bundle of size $d$ for price $\frac{d(d+1)}{2}$, i.e., paying $i$ for the $i$th item.
	For the event of $j$ non-zero items, the buyer's utility is maximized when buying all $j$ items of value $j$, with a utility of $\frac{j(j-1)}{2}$ (this bundle is in tie with the options of buying only $j-1$ of the items and having the same utility).
	The seller's expected revenue is then $1+\sum_{i=2}^{n} i\cdot\frac{1}{2i^2}$ which is logarithmic in $n$.
\end{proof}

\paragraph{symmetric for correlated is constant}\rk{is it true? if so, this is our main result...}

\paragraph{symmetric is not always amazing}(not an interesting example - marginal-symmetric requires exponential many different prices)\rk{relevant?}


